A matrix-free macro-element variant of the hybridized discontinuous Galerkin method

We investigate a macro-element variant of the hybridized discontinuous Galerkin (HDG) method, using patches of standard simplicial elements that can have non-matching interfaces. Coupled via the HDG technique, our method enables local refinement by uniform simplicial subdivision of each macro-element. By enforcing one spatial discretization for all macro-elements, we arrive at local problems per macro-element that are embarrassingly parallel, yet well balanced. Therefore, our macro-element variant scales efficiently to n-node clusters and can be tailored to available hardware by adjusting the local problem size to the capacity of a single node, while still using moderate polynomial orders such as quadratics or cubics. Increasing the local problem size means simultaneously decreasing, in relative terms, the global problem size, hence effectively limiting the proliferation of degrees of freedom. The global problem is solved via a matrix-free iterative technique that also heavily relies on macro-element local operations. We investigate and discuss the advantages and limitations of the macro-element HDG method via an advection-diffusion model problem.

==> sections/old/Conclusions_and_future_work.tex <==
\section{Conclusions and future work\label{sec:Conclusions and future work}}

==> sections/old/Governing_equations_and_test_case_description.tex <==
\section{The hybridized DG method on standard elements}

In the following, we briefly review a linear advection–diffusion equation in two and three-dimension with exact solution. We discuss the choice of the finite element spaces and the stabilization parameter, and we present the hybridization technique, which address the HDG method using on   standard elements. 
\subsection{A model problem\label{sec:Governing equations and test case description}}

As a model problem, we will use the linear advection–diffusion equations that are:

\begin{equation}\label{C21}
	\begin{split}
		\nabla \cdot\left( \mat c u\right) -\nabla \cdot\left( \kappa \nabla u\right)  & = f   \quad\quad &\text{on} \; &\Omega, \\
		u & = {{g}_{D}}    \quad\quad &\text{on} \; &\partial\Omega.\\
	\end{split} 
\end{equation}
Here, \(\Omega \subset \mathbb{R}^{d}\) is the domain in \(d\) spatial dimensions with Dirichlet boundary \(\partial \Omega\), \(u\) denotes the field solution, and \(\mat c\) and \(\mat \kappa > 0 \) are the (constant) advection and diffusion coefficients, and $f$ and ${g}_{D}$are the source term and the given solution at the Dirichlet boundary. 
Considering the auxiliary variable \(\mat q = \nabla u\), we can rewrite  Equation \eqref{C21} as a first order system of equations

\begin{equation}\label{C22}
	\begin{split}
		\mat q -\nabla u &= 0 \quad\quad &\text{on} \; &\Omega,\\
		\nabla \cdot\left( \mat{F}^{\text{adv}}\left( u\right) +\mat{F}^{\text{diff}}\left( \mat{q}\right) \right)  &=f \quad\quad &\text{on} \; &\Omega,\\
		u &= {{g}_{D}} \quad\quad &\text{on} \; &\partial\Omega,\\
	\end{split} 
\end{equation}
where the fluxes $ \mat{F}^{\text{adv}} $ and $ \mat{F}^{\text{diff}}$ are:
\begin{equation}\label{C23}
	\begin{split}
		\mat{F}^{\text{adv}}  &= \mat c u,\\
		\mat{F}^{\text{diff}} &= -\kappa \nabla u = -\kappa \mat{q}.
	\end{split} 
\end{equation}

In the following, we will derive our formulation with the help of the following two and three-dimensional test case based on  Equations (\ref{C22}, \ref{C23}), where $\Omega =\left[ 0, 1\right] ^{2}$and \(\mat c = \left( 1, 1\right)  \), and the cube $\left[ -0.5, 0.5\right] ^{3}$ for two and three-dimensional, respectively. We now choose the following exact solution: 


\begin{equation}\label{C24}
	\begin{split}
		{u}_{exact}  &=0.5 \left(1+\tanh{\left(\frac{y-2x+0.4}{\kappa}\right)} \right)        \quad\quad   &\text{for} \; & d  =  2, \\
		{u}_{exact}	 &=0.5 \left(1+\tanh{\left(\frac{x+y+z-0.5}{\kappa}\right)} \right). 	     \quad\quad   &\text{for} \; & d  = 3 
	\end{split} 
\end{equation}



We can then determine the corresponding source term $f$ and the Dirichlet boundary condition ${g}_{D}$ such that they comply with Equation \eqref{C24}. The solution regime (advection domination vs.\ diffusion domination) can be determined by the P\'{e}clet number, $\text{Pe} = \left| \mat c \right| L / \kappa$, where $L$ denotes the characteristic length scale of the domain $\Omega$, which can be modified by choosing different diffusion coefficients $\kappa$. Figure \ref{fig:test case} plots the exact solution Equation \eqref{C24} for two and three-dimensional, showing a sharp internal layer in the advection dominated regime ($\text{Pe} \gg 1$) and a slowly varying solution in the diffusion dominated regime ($\text{Pe} \approx 1$).
				
\begin{figure}
    \centering
    \subfloat[\centering Advection dominated ($\text{Pe}=\sqrt{2} \cdot10^{10}$)]{{\includegraphics[width=0.5\textwidth]{tikz/mo1e5.pdf} }}%
    \subfloat[\centering Three-dimensional]{{\includegraphics[width=0.5\textwidth]{tikz/mo1e53D.pdf} }}%
    \caption{Exact solution of the advection-diffusion model at advection dominated for two and three-dimensional.}%
    \label{fig:test case}%
\end{figure}

%The problem is a examined for accuracy order, refinement mesh and stable numerical techniques. The performance of these parameters are assessed over a large range of diffusivity, $ \kappa $, highlighting the difference between the diffusion-dominated, $ \kappa =1 $, advection-dominated limits, $ \kappa=10^{-10} $. 
%Next, we introduce the notation necessary for the description of the multi-patch coupling HDG method


==> sections/old/Implementation_aspects.tex <==
\renewcommand{\arraystretch}{1.3}
\section{Implementation aspects \label{sec:Implementation aspects}}

Up to this point, we have dealt with discretization of HDG on standard and macroelement schemes. We now summarize which discrete matrix systems are required to implement the macroelement HDG scheme to obtain a solution to the local/global variable. Another goal of this section is to describe a parallelisation strategy for macroelement HDG, which merge the strong scalability of the local linear system. We will then turn our attention to the solution of the local/global system with respect to the applicability and implementation of direct and iterative solvers.

\subsection{Linearization and local/global system of the formulation}\label{S41}

\begin{figure}
    \centering
    \subfloat[\centering $N_{i}^{Elm} = 1$ ]{{\includegraphics[width=0.33\textwidth]{tikz/A.pdf} }}%
    \subfloat[\centering $N_{i}^{Elm} = 8$ ]{{\includegraphics[width=0.33\textwidth]{tikz/A1.pdf} }}%
    \subfloat[\centering $N_{i}^{Elm} = 64$]{{\includegraphics[width=0.33\textwidth]{tikz/A2.pdf} }}%
    \caption{Sparsity pattern of the jacobian matrix Equation (\ref{C42}) in the advection–diffusion 3D problem, using $N^{Elm}=384$ with $p = 3$, and varying in $N_{i}^{Elm}$.}%
    \label{fig:PatternJacob}%
\end{figure}

To solve the macroelement HDG weak formulation, we use the Newton-Raphson method. Therefore, we have to linearize the components of the residual in Equation (\ref{C36}) at each Newton iteration. 
%\begin{equation}\label{C41}
% \begin{split}
%&\mathbf{R}_{q}(\mathbf{q}_{h},\bm{u}_{h},\widehat{\mathbf{u}}_{h}) &= 0,\\
%&\mathbf{R}_{u}(\mathbf{q}_{h},\bm{u}_{h},\widehat{\mathbf{u}}_{h}) &= 0,\\
%&\mathbf{R}_{\widehat{u}}(\mathbf{q}_{h},\bm{u}_{h},\widehat{\mathbf{u}}_{h}) &=0.
%\end{split}   
%\end{equation}
This linearization leads to solve linear systems of the form :
\begin{equation}\label{C42}
\left[ 
 \begin{array}{c | c}
\begin{matrix}  
\mathbf{A}_{qq} & \mathbf{A}_{qu}  \\  
\mathbf{A}_{uq} & \mathbf{A}_{uu} \end{matrix}   &   
\begin{matrix}  \mathbf{A}_{q \widehat{u}} \\ 
\mathbf{A}_{u \widehat{u}} \end{matrix} \\
\hline
\begin{matrix} 
\mathbf{A}_{\widehat{u} q}  & \mathbf{A}_{\widehat{u} u} \end{matrix} & 
\begin{matrix}  \mathbf{A}_{\widehat{u}  \widehat{u}} \end{matrix} 
\end{array}
\right]
 \left[ 
\begin{array}{c}
\begin{matrix}  
\delta \mathbf{q} \\  
\delta \bm{u} \end{matrix} \\ 
\hline
\begin{matrix} \delta \widehat{\mathbf{u}} \end{matrix}
\end{array}
\right]=-
 \left[ 
\begin{array}{c}
\begin{matrix}  \mathbf{R}_{q} \\  \mathbf{R}_{u} \end{matrix} \\ 
\hline
\begin{matrix} \mathbf{R}_{\widehat{u}} \end{matrix}
\end{array}
\right]
\end{equation}
where $\delta \mathbf{q}$, $\delta \mathbf{u}$ and $\delta \widehat{\mathbf{u}}$ denote the vector of updates for the coefficients of basis functions $\mathbf{q}_{h}$, $\mathbf{u}_{h}$ and $\widehat{\mathbf{u}}_{h}$, respectively. It is important to note that the degrees of freedom for $ \mathbf{q}_{h} $, $ \mathbf{u}_{h} $ are grouped together, the corresponding matrix  $[\mathbf{A}_{qq}  \mathbf{A}_{qu}; \mathbf{A}_{uq}  \mathbf{A}_{uu}]$ and $\mathbf{A}_{\widehat{u}  \widehat{u}}$ block-diagonal structure, see Figure \ref{fig:PatternJacob}. This allows us to express $\delta \mathbf{q}$ and $\delta \mathbf{u}$ in terms of $\delta \widehat{\mathbf{u}}$. For each macroelement $\mathcal{T}^{i}$, we compute the solution updates $\delta \mathbf{q}^{\mathcal{T}^{i}}$ and
 $\delta \mathbf{u}^{\mathcal{T}^{i}}$ by

\begin{equation}\label{C46}
\begin{split}
 \begin{bmatrix} 
 \delta \mathbf{q}^{\mathcal{T}^{i}} \\[7pt] 
 \delta \mathbf{u}^{\mathcal{T}^{i}}
\end{bmatrix} 
&= 
\left( \mathbf{A}_{\text{local}}^{\mathcal{T}^{i}}\right) ^{-1}\left(-\begin{bmatrix*}  
 \mathbf{R}_{q}^{\mathcal{T}^{i}} \\[7pt]   
 \mathbf{R}_{u}^{\mathcal{T}^{i}}  
\end{bmatrix*}-
\begin{bmatrix*}  
 \mathbf{A}_{q \widehat{u}}^{\mathcal{T}^{i}} \\[7pt]   
 \mathbf{A}_{u \widehat{u}}^{\mathcal{T}^{i}} 
\end{bmatrix*}
\delta \widehat{\mathbf{u}}^{\Gamma_{i}}\right) \\[7pt]
& = \begin{bmatrix} 
 \delta \mathbf{q}^{\mathcal{T}^{i}}_{\text{local}} \\[7pt] 
 \delta \mathbf{u}^{\mathcal{T}^{i}}_{\text{local}} 
\end{bmatrix} + 
 \begin{bmatrix} 
 \delta \mathbf{q}^{\mathcal{T}^{i}}_{\text{global}} \\[7pt] 
 \delta \mathbf{u}^{\mathcal{T}^{i}}_{\text{global}} 
\end{bmatrix} 
\delta \widehat{\mathbf{u}}^{\Gamma_{i}}.
\end{split}
\end{equation}
where
\begin{equation}\label{C46}
\mathbf{A}_{\text{local}}^{\mathcal{T}^{i}}
= 
\begin{bmatrix*}  
\mathbf{A}_{qq}^{\mathcal{T}^{i}} & \mathbf{A}_{qu}^{\mathcal{T}^{i}}  \\[7pt]   
\mathbf{A}_{uq}^{\mathcal{T}^{i}} & \mathbf{A}_{uu} ^{\mathcal{T}^{i}}  
\end{bmatrix*}
\end{equation}
Note, that the local update vectors $\delta \mathbf{q}^{\mathcal{T}^{i}}_{\text{local}}$ and 
$\delta \mathbf{u}^{\mathcal{T}^{i}}_{\text{local}}$, global update matrices 
$\delta \mathbf{q}^{\mathcal{T}^{i}}_{\text{global}}$ and $\delta \mathbf{u}^{\mathcal{T}^{i}}_{\text{global}}$ 
and the globally coupled reduced system of Equation (\ref{C44}) need to be stored for each macroelement.
Finally, by eliminating $\delta \mathbf{q}$ and $\delta \mathbf{u}$ from Equation (\ref{C42}), we obtain a reduced globally coupled matrix equation only for  $\delta \widehat{\mathbf{u}}$ as:
\begin{equation}\label{C44}
\widehat{\mathbf{A}}\;
\delta \widehat{\mathbf{u}}
=
\widehat{\mathbf{b}}.
\end{equation}
 The contribution to the reduced system $\widehat{\mathbf{A}}$ and residual $\widehat{\mathbf{b}}$ for each macroelement $\mathcal{T}^{i}$  are given by
\begin{equation}\label{C47}
\begin{split}
&\widehat{\mathbf{A}}^{\mathcal{T}^{i}} &= 
\mathbf{A}_{\widehat{u}  \widehat{u}}^{\mathcal{T}^{i}} -
\begin{bmatrix*}  
\mathbf{A}_{\widehat{u}q}^{\mathcal{T}^{i}} & \mathbf{A}_{\widehat{u}u}^{\mathcal{T}^{i}}
\end{bmatrix*} 
\left( \mathbf{A}_{\text{local}}^{\mathcal{T}^{i}}\right) ^{-1}
\begin{bmatrix*}  
\mathbf{A}_{q \widehat{u}}^{\mathcal{T}^{i}} \\[7pt]
 \mathbf{A}_{u \widehat{u}}^{\mathcal{T}^{i}}
\end{bmatrix*},\\[7pt]
&\widehat{\mathbf{b}}^{\mathcal{T}^{i}} &= 
-\mathbf{R}_{\widehat{u}}^{\mathcal{T}^{i}} -
\begin{bmatrix*}  
\mathbf{A}_{\widehat{u}q}^{\mathcal{T}^{i}} & \mathbf{A}_{\widehat{u}u}^{\mathcal{T}^{i}}
\end{bmatrix*} 
\left( \mathbf{A}_{\text{local}}^{\mathcal{T}^{i}}\right) ^{-1}
\begin{bmatrix*}  
 \mathbf{R}_{q}^{\mathcal{T}^{i}} \\[7pt] 
 \mathbf{R}_{u}^{\mathcal{T}^{i}}
\end{bmatrix*}.
\end{split}
\end{equation}

Finally, due to assembling these contributions, we obtain $\widehat{\mathbf{u}}$ by solving the linear system in Equation (\ref{C44}).
This is the global system to be solved at every Newton iteration. Since $\widehat{\mathbf{u}}_{h}$ is defined and single-valued along the faces, the final matrix system of the HDG method is smaller than that of many other DG methods  \cite{cockburn2016static, peraire2010hybridizable, nguyen2015class}. Moreover, the matrix $\widehat{\mathbf{A}}$ is compact in the sense that only the degrees of freedom between neighboring the faces that share the same element are connected \cite{peraire2010hybridizable}.


If we also take a look at the sparsity pattern varying of $N_{i}^{Elm}$ in Figure \ref{fig:PatternJacob}, we observe what should already be clear from the construction of the method: On the one hand standard HDG  methods, in comparison to macroelement HDG methods, come with additional local/global degrees of freedoms, but on the other hand the stencil of the formulation is reduced and so the coupling of degrees of freedom is reduced. 

We observe that the number of the local matrix decreases, but the size of the local matrix increases when we increase the $N_{i}^{Elm}$. We additionally remark that the advantage of macroelement HDG method is that the resulting local system, $\mathbf{A}_{\text{local}}^{\mathcal{T}^{i}}$, enjoys greater sparsity in Figure \ref{fig:PatternJacob}(c).

\subsection{Distributed and parallel implementation}\label{S43}
The parallel implementation of the HDG on macroelement method here is straightforward and summarized in Algorithm 1. In practice, we compute the vector of updates $\delta \mathbf{q}$, $\delta \mathbf{u}$ and $\delta \widehat{\mathbf{u}}$ from $\mathbf{q}_{h}$, $\mathbf{u}_{h}$ and $\widehat{\mathbf{u}}_{h}$. Line 4, in which the matrix contributions are distributed from the macroelement,$\mathcal{T}^{i}$ ,to process $n$. For obtaining that their components, we require only local data from each processor, $\mathcal{T}_{h}^{n}$, due to the discontinuous nature of macroelements, and hence requires no communication between processors. Then, the distributed global matrix $\widehat{\mathbf{A}}$ and vector $\widehat{\mathbf{b}}$ are computed from locally  $\widehat{\mathbf{A}}^{\mathcal{T}^{i}}$ and $\widehat{\mathbf{b}}^{\mathcal{T}^{i}}$, Lines 2-7. The global linear system solve referenced in Line 8 refers to an iterative solution procedure such as restarted Generalized Minimal Residual (GMRES) method \cite{{saad1986gmres}}. Finally, the obtained value of $\delta \widehat{\mathbf{u}}$ allows obtaining $\delta \mathbf{q}$ and $\delta \mathbf{u}$ in an element-wise manner, Lines 9-14. 

Note, that all the previous loops can be performed in parallel, as these operations are completely independent on each macroelement. Specifically, the computation of the macroelement: the local linear systems, inverses in Equation (\ref{C46}), and the global linear systems in Equation (\ref{C47}). The main advantage of this parallelization macroelement HDG scheme is that the computational balance changes towards the local solver. Therefore, the effect of global linear solver in the total time is lessened, and the result is a more weak and strong scalability. In Section (\ref{S5.1.1}) and Section (\ref{S5.2.1}), we numerically study the effects of parallelizing these methods.

\begin{algorithm}
\caption{Distributed solver for the macroelement discretization}
\begin{algorithmic}[1]

\State $ n \gets$ Current processor
\Procedure  {Compute distributed global system} {$\widehat{\mathbf{A}}$ and $\widehat{\mathbf{b}}$ from $\mathbf{q}$, $\mathbf{u}$, $\widehat{\mathbf{u}}$}
\For {$\mathcal{T}^{i} \in \mathcal{T}_{h}^{n}$}
\State $\widehat{\mathbf{A}}^{\mathcal{T}^{i}}, \widehat{\mathbf{b}}^{\mathcal{T}^{i}} \gets$ 
Matrix contributions from $\mathbf{q}^{\mathcal{T}^{i}}$, $\mathbf{u}^{\mathcal{T}^{i}}$, $\widehat{\mathbf{u}}^{\Gamma_{i}}$
\State $\widehat{\mathbf{A}}, \widehat{\mathbf{b}} \gets$ 
Assemble $\widehat{\mathbf{A}}^{\mathcal{T}^{i}}$ and $\widehat{\mathbf{b}}^{\mathcal{T}^{i}}$ for all $\mathcal{T}^{i} \in \mathcal{T}_{h}^{n}$
\EndFor
\EndProcedure


\State $\delta \widehat{\mathbf{u}} \gets$ Solve $\widehat{\mathbf{A}}\;\delta \widehat{\mathbf{u}}=\widehat{\mathbf{b}}$

\Procedure  {Compute distributed local system} {obtain $\delta {\mathbf{q}}$ and $\delta {\mathbf{u}}$ from $\delta\widehat{\mathbf{u}}$}
\For {$\mathcal{T}^{i} \in \mathcal{T}_{h}^{n}$}
\State ${\delta\mathbf{q}}^{\mathcal{T}^{i}},{\delta\mathbf{u}}^{\mathcal{T}^{i}} \gets$ 
Reconstruct elemental solution from $\delta  \widehat{\mathbf{u}}^{\Gamma_{i}}$ 
\State ${\delta \mathbf{q}},{\delta \mathbf{u}} \gets$ 
Assemble ${\delta\mathbf{q}}^{\mathcal{T}^{i}}$ and ${\delta\mathbf{u}}^{\mathcal{T}^{i}} $ for all $\mathcal{T}^{i} \in \mathcal{T}_{h}^{n}$
\EndFor
\EndProcedure

\end{algorithmic}
\end{algorithm}

\subsection{Solving the local/global linear system}

\begin{figure}
    \centering
    \subfloat[\centering $N_{i}^{Elm} = 1$ ]{{\includegraphics[width=0.33\textwidth]{tikz/Ahs.pdf} }}%
    \subfloat[\centering $N_{i}^{Elm} = 8$ ]{{\includegraphics[width=0.33\textwidth]{tikz/Ahs1.pdf} }}%
    \subfloat[\centering $N_{i}^{Elm} = 64$]{{\includegraphics[width=0.33\textwidth]{tikz/Ahs2.pdf} }}%
    \caption{Sparsity pattern of the global matrix Equation (\ref{C44}) in the advection–diffusion 3D problem with the reverse Cuthill–McKee reordering, using $N^{Elm}=384$ with $p=3$, and varying in $N_{i}^{Elm}$}%
    \label{fig:PatternGBL}%
\end{figure}


The linear system that arise from HDG weak formulation, Section (\ref{S41}), can be solved in two stages: solving the global linear system and solving the local linear system.

The local linear system is solved directly using the LU factorisation and sparse format matrices. Moreover, as macroelement size grows, the factorization time begins to dominate the time-to-solution. So, the storage and application of $\left( \mathbf{A}_{\text{local}}^{\mathcal{T}^{i}}\right) ^{-1}$ has important implications for macroelement HDG schemes. Note that application of the local matrix in each macroelement as a dense array is inefficient; generally, 3D problems at degrees of freedoms per patch $\text{dof}^{local}_{i} \geqslant 100$  tend to be sparse. Storing the complete, fully-dense local matrix would be wasteful. Therefore, a sparse representation of $\mathbf{A}_{\text{local}}^{\mathcal{T}^{i}}$ can be applied much more efficiently. Before assembling the matrix, we reorder using the reverse Cuthill-McKee (RCM) algorithm \citep{liu1976comparative} to reduce the bandwidth of the system and the resulting factorisation. We have found that this combination of sparse format and RCM is efficient for macroelement HDG methods, especially when the $\text{dof}^{local}_{i}$ increases due to higher $N_{i}^{Elm}$. 




For solving the global linear system, we used a iterative solvers to the solution of the global linear system $\widehat{\mathbf{A}}\;\delta \widehat{\mathbf{u}}=\widehat{\mathbf{b}}$. Note that the patch partition used to distribute the problem determined the domains of the decomposition for the global system. In order to give a qualitative idea of how the macroelement size may affects performance of global solver, in Figure \ref{fig:PatternGBL} we compare the rank and sparsity pattern of global matrix for the standard HDG method compared to the HDG on macroelement method as a function of $N_{i}^{Elm}$. We observe from the standard HDG to macroelement HDG that macroelement with $N_{i}^{Elm}=64$ leads to a smaller rank and larger bandwidth global system. Despite the higher rank of the HDG on standard element approach the weaker elemental coupling of the technique leads to a reduced matrix bandwidth and faster compute time of preconditioner when using incomplete LU factorization. We will introduce these properties by performing a several of numerical experiments to determine the weak and strong scalability of each method in Section (\ref{sec: Numerical and performance results}).

\subsection{Local adaptive refinement }

In this study, we are interested in using locally refined elements. Four-way and eight-way refinement procedure used based on same element for 2D and 3D, respectively. Since, we want to build $\widehat{u}_{h}$’s continuity into its space, refinement elements will result in a nonconforming skeleton space. The $\widehat{u}_{h}$-space is defined by the span of basis functions of the fine side and apply a constraint to guarantee the continuity. Based on, we enforce continuity in the skeleton space for $\widehat{u}_{h}$, and obtain an efficient hybrid method which also has the flexibility of discontinuous Galerkin methods \citep{samii2016parallel}.

At this point in time, we want to evaluate the behavior of the adaptive refinement algorithm. For this regards, We consider the test case presented in Section (\ref{sec:Governing equations and test case description}) with $k=10^{-10}$. This leads to a internal layer at the domain, see Figure \ref{fig:test case}(a), which involves very high gradients in the solution. But instead of a uniform refinement of the macroelement, we refine the macroelement according to the internal layer. Employing an automatic refinement scheme, we obtain a sequence of triangular meshes, starting from a $N^{ptch}=50$ with $N^{Elm}_{i}=4$ mesh, shown in Figure \ref{fig:Mesh refine} that capture the location of the internal layers very well.
\begin{figure}
    \centering
     \subfloat[\centering refinement of level 1.]{{\includegraphics[width=0.33\textwidth]{tikz/ref2.pdf} }}%
     \subfloat[\centering refinement of level 2.]{{\includegraphics[width=0.33\textwidth]{tikz/ref2.pdf} }}%
     \subfloat[\centering refinement of level 3.]{{\includegraphics[width=0.33\textwidth]{tikz/ref3.pdf} }}\\ %%
     \subfloat[\centering refinement of level 4.]{{\includegraphics[width=0.33\textwidth]{tikz/ref4.pdf} }}%
     \subfloat[\centering refinement of level 5.]{{\includegraphics[width=0.33\textwidth]{tikz/ref5.pdf} }}%
     \subfloat[\centering refinement of level 6.]{{\includegraphics[width=0.33\textwidth]{tikz/ref6.pdf} }} 
    \caption{Sequence of patches pattern generated by a refinement scheme for advection–diffusion 2D problem whit $k=10^{-10}$.}%
    \label{fig:Mesh refine}%
\end{figure}
\begin{table}
\caption{Number of local and global unknowns and elements in the advection–diffusion 2D problem with $k=10^{-10}$ of different local level refinement.} 
\centering
\begin{tabular}{llllllllll} 
 \hline
 Size/Level 				&  1 		 & 2 		&  3			&  4  		& 5			& 6 				& 7 			&8				& 9\\ 
  \hline
 $N^{Elm}$ 				& 200  		 & 380  		& 740  		& 1,460  	& 2,900 		& 5,780 			&11,540 		&30,740			&99,860 \\  
 $\text{dof}^{global}$ 	& 510	 	 & 954  		& 1,836  	& 3,588 	 	& 7,080 		&14,052  		&27,984  	&73,116			&233,454 \\ 
 $\text{dof}^{local}$ 	& 2,250 		 & 4,275 	& 8,325  	& 16,425  	& 32,625 	& 65,025 		&129,825 	&345,825			&1,123,425 \\
 \hline
\end{tabular}
\label{Tab:Adaptive mesh}%
\end{table}

The number of local and global unknowns and elements with increasing levels of adaptive refinement are illustrated in Table \ref{Tab:Adaptive mesh}. Also, in Figure \ref{fig:convergence refine}, the convergence plots of $u_{h}$ in $p=2$ for different refinements are presented. Due to the uniformity and smoothness of the solution, one should not expect an optimal convergence from the adaptive refinement. However, the comparison of adaptive and uniform demonstrates that adaptive refinement leads to a  similar optimal convergence rate.
 \begin{figure}
    \centering
     \subfloat[\centering Convergence of uniform and adaptive refinement.]{{\includegraphics[width=0.55\textwidth]{tikz/convergref.pdf} }}%
     \subfloat[\centering Solution obtained refinement level 9.]{{\includegraphics[width=0.45\textwidth]{tikz/Uref.pdf} }}
    \caption{Convergence of advection–diffusion 2D problem whit $k=10^{-10}$ and $p=2$.}%
    \label{fig:convergence refine}%
\end{figure}



 
 
 
 
 
 
\subsection{Scaling of the local system}
In this section, the description of the strong scalability of local system that using the parallel macroelement HDG solver for uniform triangle mesh with the diffusivity, $k=1$ are presented. In Table \ref{Tab:p2 and2D element size}, one mesh with different interpolation degree, number of local and global unknowns, and local unknowns per macroelement have been generated. For study the execution local time of different patch size, the computation time for the $N^{Elm}=51,200$ elements of two orders, $p=2$ and $p=3$, are presented in Table \ref{Tab:p2 and 2D scaling}. Furthermore, the local time in varying of $N_{i}^{Elm}$ are also listed in this table. As mentioned, by local computations, we mean the inverses, assemble local matrix and calculate the local values computation from global solution. The direct sparse LU factorization (UMFPACK \cite{davis2004algorithm}) is considered for solving the local matrix. These results were obtained on seven node of the cluster system of Leibniz University Hannover (LUH), which has 32 processes per node. In order to examine the performance, Figure \ref{fig:2D Scaling} shows also the computation speedups corresponding to each case. Speedup characterizes the amount of performance gain using $n\geqslant32$ cores, and is defined as follows:
 
 \begin{align*}
    S_{n} = \frac{\text{Elapsed time using 32 cores}}{\text{Elapsed time using n cores}}.       
\end{align*}

Also, the computation efficiency using $n$ cores is defined as $E_{n}= S_{n}/n$. This observation demonstrates that the parallel local solver is significantly scalable, see Figure \ref{fig:2D Scaling}. It is worthwhile noting that, for varying in $N_{i}^{Elm}$, we have obtained an efficiency between $87\%$ to $99\%$.


 \begin{table}
\caption{Number of local and global unknowns and local unknowns per patch in the advection–diffusion 2D problem, using $N^{Elm}=51,200$ with $p=2-3$, and varying in $N_{i}^{Elm}$.} 
\centering
\begin{tabular}{lllllll}\toprule
& \multicolumn{3}{c}{$p = 2$} & \multicolumn{3}{c}{$p = 3$} 
\\\cmidrule(lr){2-4}\cmidrule(lr){5-7}
          & $N_{i}^{Elm} =1$   & $N_{i}^{Elm} =16$  & $N_{i}^{Elm} =64$ 	& $N_{i}^{Elm} =1$   & $N_{i}^{Elm} =16$  & $N_{i}^{Elm} =64$ \\\midrule           
 $\text{dof}^{local}$  			&921,600  	&432,000 	&367,200		&1,536,000  			 		    &873,600 					&780,000\\[5pt]
 $\text{dof}^{global}$ 			&231,360 	&43,920 		&21,080		&308,480	 	 	 	 			&63,440 			    			&3,1000\\[5pt]
 $N^{ptch}$ 	 					&51,200  	&3,200  		&800			&51,200  		 	 			&3,200  						&800\\[5pt]
 $\text{dof}^{local}_{i}$   		&40  		&140 		&660			&30  		 	 			 	&273 						&975\\\bottomrule
\end{tabular}
\label{Tab:p2 and2D element size}%
\end{table}




 \begin{table}
\caption{Execution the local computations time(s) in the advection–diffusion 2D problem, using $N^{Elm}=51,200$ with $p = 2-3$, and varying in $N_{i}^{Elm}$.} 
\centering
\begin{tabular}{lcccccc}\toprule
& \multicolumn{3}{c}{$p = 2$} & \multicolumn{3}{c}{$p = 3$} 
\\\cmidrule(lr){2-4}\cmidrule(lr){5-7}
          & $N_{i}^{Elm} =1$   & $N_{i}^{Elm} =16$  & $N_{i}^{Elm} =64$ 	& $N_{i}^{Elm} =1$   & $N_{i}^{Elm} =16$  & $N_{i}^{Elm} =64$ \\\midrule           
 $Cores = 32$  			&2.27	&3.06	&13.25	&2.76	&14.39	&139.74\\
 $Cores = 64$  			&1.17	&1.63	&7.44	&1.41	&7.74	&87.32\\
 $Cores = 96$  			&0.78	&1.06	&4.79	&0.96	&5.16	&55.28\\
 $Cores = 128$  			&0.58	&0.80	&3.52	&0.73	&3.87	&37.87\\
 $Cores = 160$  			&0.47	&0.63	&2.80	&0.58	&3.03	&29.80\\
 $Cores = 192$  			&0.39	&0.52	&2.31	&0.48	&2.53	&24.86\\
 $Cores = 224$			&0.33	&0.43	&1.77	&0.41	&2.09	&18.43\\\bottomrule
\end{tabular}
\label{Tab:p2 and 2D scaling}%
\end{table}
 
  \begin{figure}
    \centering
     \subfloat[\centering Scaling of local solver with $p = 2$.]{{\includegraphics[width=0.5\textwidth]{tikz/localp2.pdf} }}%
     \subfloat[\centering Scaling of local solver with $p = 3$.]{{\includegraphics[width=0.5\textwidth]{tikz/localp3.pdf} }}
    \caption{Strong scaling of advection–diffusion 2D problem, using $N^{Elm}=51,200$ with $p = 2, 3$, and varying in $N_{i}^{Elm}$.}%
    \label{fig:2D Scaling}%
\end{figure}
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 



==> sections/old/Multi-Patch_Coupling_HDG_Method.tex <==
%\section{Multi-patch coupling HDG method\label{sec:/Multi-patch coupling HDG method}}

\subsection{Discontinuous finite element spaces}\label{space HDG}

%\subsubsection{Finite element mesh}
We denote by \({\mathcal{T}}_{h}\) a collection of elements \(K\) that partition \(\Omega\), and set \(\partial \mathcal{T}_{h} := \left\lbrace  \partial K: K \in \mathcal{T}_{h} \right\rbrace \)  to be the collection of the boundaries of the elements in \({\mathcal{T}}_{h}\).
For an element \(K\), \(e =\partial K  \cap \partial \Omega\) is a boundary face. % if its \(d-1\) Lebesgue measure is nonzero. 
For two elements \({K}^{+}\) and \({K}^{-}\) of \({\mathcal{T}}_{h}\),  \(e =\partial {K}^{+}  \cap \partial {K}^{-}\) is the interior face between  \({K}^{+}\)  and  \({K}^{-}\). %  if its  \(d-1\) Lebesgue measure is nonzero. 
We denote by \({\varepsilon}^{Int}\) and \({\varepsilon}^{\partial}\) the set of interior and boundary faces, respectively, and we define
 \({\varepsilon}_{h} :={ \varepsilon}^{Int} \cup {\varepsilon}^{\partial}\) 
 as the union of interior and boundary faces.

We denote by $ \mathcal{P}^{p}\left( D\right)  $ the set of polynomials of degree $p$ on a domain $D$ and let $ L^{2}\left( D\right)  $ be the space of square-integrable functions on $D$. For any element $K$ of the collection $\mathcal{T}_{h}$ we denote $\mathcal{V}^{p}\left(K\right) \equiv \mathcal{P}^{p}\left(K\right)$ and $\bm{\mathcal{Q}}^{p}\left(K\right) \equiv \left( \mathcal{P}_{p}\left(K\right)\right) ^{d}$. We can now introduce the following discontinuous finite element spaces:
\[\mathcal{V}^{p}_{h} 
 = \left\lbrace  v \in L^{2}\left( \mathcal{T}_{h} \right) :  
 v\mid_{K} \in \mathcal{V}^{p}\left(K\right), \; \;\; \forall K  \in \mathcal{T}_{h} \right\rbrace ,\]
\[\bm{\mathcal{Q}}^{p}_{h} 
 = \left\lbrace  \bm{w} \in [L^{2}\left(\mathcal{T}_{h}\right)]^{d} : 
 \bm{w}\mid_{K} \in \bm{\mathcal{Q}}^{p}\left(K\right), \;\;\; \forall K  \in \mathcal{T}_{h} \right\rbrace .\]
 
 
 Moreover, we introduce the following finite element spaces for a traced finite element space:
\[\mathcal{M}^{p}_{h} = \left\lbrace  \mu \in L^{2}\left( \varepsilon_{h}\right)   : 
 \mu\mid_{e} \in \mathcal{P}^{p}\left( e\right),  \;\;\; \forall e  \in \varepsilon_{h} \right\rbrace ,\]
 
Next, we define several inner products associated with these finite element spaces. In particular, defined $ w,v$ on $\mathcal{T}_{h}$, $ \varphi,\psi$ on $\partial\mathcal{T}_{h}$, and $ \eta,\zeta$ on ${\varepsilon}_{h}$, we write







\begin{equation}\label{C31}
 \begin{split}
&\left( w,v\right) _{\mathcal{T}_{h}}= \sum_{K\in\mathcal{T}_{h}}\left( w,v\right) _{K}= \sum_{K\in\mathcal{T}_{h}}\int_{K} w\cdot v,\\
&\left\langle \varphi,\psi\right\rangle_{\partial\mathcal{T}_{h}}= \sum_{K\in\mathcal{T}_{h}}\left\langle \varphi,\psi\right\rangle_{\partial K}
= \sum_{K\in\mathcal{T}_{h}}\int_{\partial K} \varphi\cdot\psi.\\
 \end{split} 
\end{equation} 
And, the corresponding inner product for functions in the trace spaces:
\begin{equation}\label{C32}
 \begin{split}
&\left\langle \eta,\zeta\right\rangle_{{\varepsilon}_{h}}= \sum_{e\in{\varepsilon}_{h}}\left\langle \eta,\zeta\right\rangle_{e}.
  \end{split} 
\end{equation} 
for all $ \eta,\zeta\in \mathcal{M}^{p}_{h} $.

\subsection{Element-wise discretization}
Following previous work on HDG methods \cite{cockburn2009hybridizable, nguyen2009implicit}, the strong form given by Equation (\ref{C22}) is solved in two stages.
First, multiplying the first two Equations (\ref{C22}) by test functions and integrating by parts, we seek an approximation $\left(\mathbf{q}_{h}, {u}_{h} \right)\in \bm{\mathcal{Q}}^{p}_{h} \times \mathcal{V}^{p}_{h}$ such that for all $K \in \mathcal{T}_{h}$, 


\begin{equation}\label{C33}
 \begin{split}
&\left( \mathbf{q}_{h},\bm{w}\right) _{K} + \left( {u}_{h},\nabla\cdot\bm{w}\right) _{K} -\left\langle  \widehat{u}_{h} ,\bm{w}\cdot\bm{n}\right\rangle  _{\partial K} &= 0,	\quad
&\forall \bm{w} \in \left( \mathcal{P}_{p}\left( K\right) \right) ^{d},\\
&\left( \mathbf{F}_{h}^{\text{adv}} + \mathbf{F}_{h}^{\text{diff}},\nabla v\right) _{K} - 
\left\langle  \left( \widehat{\mathbf{F}}_{h}^{\text{adv}}+\widehat{\mathbf{F}}_{h}^{\text{diff}}\right) \cdot\bm{n},v \right\rangle  _{\partial K} - \left( f,v\right) _{K}&= 0, \quad
&\forall v \in \mathcal{P}_{p}\left( K\right) .  
\end{split} 
\end{equation}
where $ \bm{n} $ is the outward unit normal vector. Second, by adding the Equation (\ref{C33}) over all the elements and imposes the continuity of the normal component of the  total  numerical  flux \cite{cockburn2009hybridizable}. Find $ \left( \mathbf{q}_{h}, u_{h},\widehat{u}_{h}\right) \in \bm{\mathcal{Q}}^{p}_{h} \times \mathcal{V}^{p}_{h} \times \mathcal{M}^{p}_{h}$ such that
\begin{subequations}
 \begin{align}
&\left( \mathbf{q}_{h},\bm{w}\right) _{\mathcal{T}_{h}} + \left( {u}_{h},\nabla\cdot\bm{w}\right) _{\mathcal{T}_{h}} - \left\langle  \widehat{u}_{h} ,\bm{w}\cdot\bm{n}\right\rangle  _{\partial \mathcal{T}_{h}} &= 0,	\quad 
&\forall \bm{w} \in \bm{\mathcal{Q}}^{p}_{h},\label{C34A}\\
&\left(\mathbf{F}_{h}^{\text{adv}} + \mathbf{F}_{h}^{\text{diff}},\nabla v\right) _{\mathcal{T}_{h}} - 
\left\langle  \left( \widehat{\mathbf{F}}_{h}^{\text{adv}}+\widehat{\mathbf{F}}_{h}^{\text{diff}}\right) \cdot\bm{n},v \right\rangle  _{\partial \mathcal{T}_{h}} - \left( f,v\right) _{\mathcal{T}_{h}}&= 0,	\quad &\forall v \in \mathcal{V}^{p}_{h},\label{C34B} \\
&\left\langle  \left( \widehat{\mathbf{F}}_{h}^{\text{adv}}+\widehat{\mathbf{F}}_{h}^{\text{diff}}\right) \cdot\bm{n},\mu\right\rangle  _{{\varepsilon}_{h}\backslash\partial\Omega} 
 + \left\langle  \widehat{b}_{h},\mu\right\rangle  _{\partial\Omega}&= 0,	\quad &\forall \mu \in \mathcal{M}^{p}_{h}. \label{C34C} 
 \end{align}
\end{subequations}
Note that the boundary trace operator, $ \widehat{b}_{h}\left( \widehat{u}_{h},u_{h},\mathbf{q}_{h}\right) $, is imposed the boundary conditions along $\partial\Omega $ on the numerical trace.
\[\widehat{b}_{h}\left( \widehat{u}_{h},u_{h},\mathbf{q}_{h}\right)  =  \widehat{u}_{h}-g_{D}\]

Now, we define the fluxes at the interfaces that appear after the integration by parts due to the discontinuous nature of the approximation spaces are chosen as:
\begin{equation}\label{C35}
 \begin{split}
&\widehat{\mathbf{F}}_{h}^{\text{adv}}\cdot\bm{n} = 
\mathbf{c}\widehat{u}_{h}\cdot\bm{n}+
\tau_{\text{adv}}\left( u_{h}-\widehat{u}_{h}\right)  \;\;\;\; &&on \; \partial K\\
&\widehat{\mathbf{F}}_{h}^{\text{diff}}\cdot\bm{n} = 
-\kappa\mathbf{q}_{h}\cdot\bm{n} +
\tau_{\text{diff}}\left( u_{h}-\widehat{u}_{h}\right)  \;\;\;\; &&on \; \partial K
\end{split}   
\end{equation}
in the above expressions, $ \tau_{\text{adv}} $ and $ \tau_{\text{diff}} $ present a stabilization parameter of the advection and diffusive component, such as 
\[\tau_{\text{adv}} = \vert \bm{c}\cdot \bm{n}\vert,\;\;\;\; \tau_{\text{diff}} = k/l \]
where $ l $ is a typical length scale of the problem. For more details see \cite{cockburn2009unified, cockburn2009superconvergent}. 

On the one hand, we insert the numerical normal traces from Equation (\ref{C35}) into Equations (\ref{C34B}) and (\ref{C34C}), and  obtain leads to the semi-discrete locally, Equation (\ref{C34A})  and (\ref{C34B}), and globally problems, Equation (\ref{C34C}).


\section{The hybridized DG method on macroelement patches\label{sec:/Multi-patch coupling HDG method}}

We start with a notation and finite element spaces and show how this spaces can be deploy to macroelements HDG method, which combines continuous and discontinuous. We introduce basic ideas and discretization of the HDG on macroelement method. The concept of SUPG stabilization can also be apply to this scheme, which we illustrate a beneficial effect on stabilization with a simple advection–diffusion example in two dimension. We conclude with an examples of hybridized DG on macroelement methods are presented, and a comparison with
standard HDG methods in two/three dimensions. 

\subsection{Finite element mesh on macroelement}\label{S330}

Let the physical domain be the union of $ N^{ptch} $ isogeometric patches (macroelement), i.e  such that $ \overline{\Omega}=\cup^{N^{ptch}}_{i=1}\overline\Omega_{i}$ and $ \Omega_{i}\cap\Omega_{j}=\varnothing$ for $ i\neq j $. The patches $ \Omega_{i} $ are consisting of a union of elements in $ \mathcal{T}_{h}  $. 
We also denote by $ \mathcal{T}_{i} $ a union of elements that satisfies $ \mathcal{T}_{i} \subseteq \mathcal{T}_{h}$. The interface of subdomain $ \Omega_{i} $ is defined as $\Gamma_{i}=\partial\Omega_{i} $ while the collection of patch interfaces $ \Gamma $ is defined as $ \Gamma=\cup^{N^{ptch}}_{i=1} \Gamma_{i}$. The domain $ \Omega $ is partitioned into $ N^{ptch} $ macroelements, a total of $ N^{Elm} $ standard elements, and each macroelement consists of $ N_{i}^{Elm} = N^{Elm}/N^{ptch} $ elements. In HDG on standard element method, we have  $ N^{Elm} =  N^{ptch} $ and $ N_{i}^{Elm} = 1$.


\subsection{Finite element spaces on macroelement}\label{S330}

\subsubsection{Finite element spaces on local variable}
\begin{figure}
    \centering
     \subfloat[\centering Standard element HDG.]{{\includegraphics[width=0.33\textwidth]{tikz/SHDG.pdf} }}%
     \subfloat[\centering Macroelement HDG.]{{\includegraphics[width=0.33\textwidth]{tikz/MHDG.pdf} }}%
     \subfloat[\centering Continuous Galerkin.]{{\includegraphics[width=0.33\textwidth]{tikz/CG.pdf} }}\\ %% 
    \caption{Illustration of the degrees of freedom for the standard HDG, macroelement HDG and CG methods. The blue line represent the boundary of the macroelemets, while the black line represent the boundary of the standard elements.}%
    \label{fig:SHDG MHDG CG}%
\end{figure}


In addition to the notation introduced in Section (\ref{space HDG}), we need to define a new approximation space as
\begin{equation}
 \begin{split}
 &\widehat{\mathcal{V}}^{p}_{h} 
 = \left\lbrace  v \in C^{0}\left( \mathcal{T}_{h}\right)  :  
 v \mid_{K} \in \mathcal{P}^{p}\left( K\right)  \; \;\; \forall K  \in \mathcal{T}_{h} \right\rbrace ,\\
&\widehat{\bm{\mathcal{Q}}}^{p}_{h} 
 = \left\lbrace  \bm{w} \in C^{0}\left( \mathcal{T}_{h}\right) ^{d} : 
 \bm{w} \mid_{K} \in [\mathcal{P}^{p}\left( K\right) ]^{d} \;\;\; \forall K  \in \mathcal{T}_{h} \right\rbrace ,
 \end{split} 
\end{equation} 
where $ C^{0}(D) $ is the space of continuous functions on $ D $. Note that $ \mathcal{V}^{p}_{h}  $ and $ \bm{\mathcal{Q}}^{p}_{h}  $ consist of
functions which are discontinuous at the boundaries of the elements, whereas $ \widehat{\mathcal{V}}^{p}_{h}  $ and $ \widehat{\bm{\mathcal{Q}}}^{p}_{h} $ consist of functions that are continuous at the boundaries of the elements. We also denote by $\widetilde{\mathcal{V}}^{p}_{h}$ and $\widetilde{\bm{\mathcal{Q}}}^{p}_{h}$ a finite element space that satisfies 
$\widehat{\mathcal{V}}^{p}_{h} \subseteq \widetilde{\mathcal{V}}^{p}_{h} \subseteq \mathcal{V}^{p}_{h}$ 
and  
$\widehat{\bm{\mathcal{Q}}}^{p}_{h} \subseteq \widetilde{\bm{\mathcal{Q}}}^{p}_{h} \subseteq \bm{\mathcal{Q}}^{p}_{h}$. In particular, we define 

\begin{equation}
 \begin{split}
 &\widetilde{\mathcal{V}}^{p}_{h} 
 = \left\lbrace  v \in L^{2}\left( \mathcal{T}_{h}\right)  :  
 v \mid_{K} \in \mathcal{P}^{p}\left( K\right)  \; \;\; \forall K  \in \mathcal{T}_{h}  \;\;\; \text{and}  \;\;\; v \mid_{\mathcal{T}^{i}_{h}} \in C^{0}\left( \mathcal{T}^{i}_{h}\right) \right\rbrace ,\\
&\widetilde{\bm{\mathcal{Q}}}^{p}_{h} 
 = \left\lbrace  \bm{w} \in L^{2}\left( \mathcal{T}_{h}\right) ^{d} : 
 \bm{w} \mid_{K} \in [\mathcal{P}^{p}\left( K\right) ]^{d} \;\;\; \forall K  \in \mathcal{T}_{h}  \;\;\; \text{and}  \;\;\; \bm{w} \mid_{\mathcal{T}^{i}_{h}} \in C^{0}\left( \mathcal{T}^{i}_{h}\right)^{d} \right\rbrace ,
 \end{split} 
\end{equation} 
where $\mathcal{T}^{i}_{h}$ is a subset of $\mathcal{T}_{h}$. Note that $\widetilde{\mathcal{V}}^{p}_{h}$ and $\widetilde{\bm{\mathcal{Q}}}^{p}_{h}$ consist of functions which are continuous on the inside macroelement,$\mathcal{T}^{i}_{h}$, and  discontinuous on the boundaries of the macroelements. Furthermore, if $\mathcal{T}^{i}_{h} = \mathcal{T}_{h}$ then $\widetilde{\mathcal{V}}^{p}_{h}=\widehat{\mathcal{V}}^{p}_{h} $ and $\widetilde{\bm{\mathcal{Q}}}^{p}_{h}=\widehat{\bm{\mathcal{Q}}}^{p}_{h}$ and if $\mathcal{T}^{i}_{h} = K$ then $\widetilde{\mathcal{V}}^{p}_{h} = \mathcal{V}^{p}_{h}$ and $\widetilde{\bm{\mathcal{Q}}}^{p}_{h} = \bm{\mathcal{Q}}^{p}_{h}$. 

Hence, different choices of $\mathcal{T}^{i}_{h}$ lead to different schemes within the hybridized DG family. We briefly discuss three important choices of $\mathcal{T}^{i}_{h}$. The first one is $\mathcal{T}^{i}_{h} = K$ and implies $\widetilde{\mathcal{V}}^{p}_{h} = \mathcal{V}^{p}_{h}$ and $\widetilde{\bm{\mathcal{Q}}}^{p}_{h} = \bm{\mathcal{Q}}^{p}_{h}$. This choice corresponds to the hybridizable discontinuous Galerkin (HDG) method on standard element \cite{cockburn2009unified}. The second choice is $\mathcal{T}^{i}_{h} = \mathcal{T}_{h}$ which implies $\widetilde{\mathcal{V}}^{p}_{h}=\widehat{\mathcal{V}}^{p}_{h}$ and  $\widetilde{\bm{\mathcal{Q}}}^{p}_{h}=\widehat{\bm{\mathcal{Q}}}^{p}_{h}$, thus enforces the continuity of the approximate unknowns on all elements. This choice corresponds to the continuous Galerkin (CG) method introduced in \cite{hughes2012finite,kirby2012cg}. Since $\widehat{\mathcal{V}}^{p}_{h} \subseteq \mathcal{V}^{p}_{h}$ and $\widehat{\bm{\mathcal{Q}}}^{p}_{h} \subseteq \bm{\mathcal{Q}}^{p}_{h}$, the CG method has fewer locally coupled degrees of freedom that the HDG method \cite{yakovlev2016cg}. And the third choice of the approximation spaces of locally unknowns are obtained by setting $K \subset \mathcal{T}^{i}_{h} \subset \mathcal{T}_{h}$, which implies $\widehat{\mathcal{V}}^{p}_{h} \subset \widetilde{\mathcal{V}}^{p}_{h} \subset \mathcal{V}^{p}_{h}$ and $\widehat{\bm{\mathcal{Q}}}^{p}_{h} \subset \widetilde{\bm{\mathcal{Q}}}^{p}_{h} \subset \bm{\mathcal{Q}}^{p}_{h}$. The resulting approximation spaces consist of functions which are discontinuous over the union of the boundary locally DOFs and continuous over the union of the interior locally DOFs of the macroelements $\mathcal{T}^{i}_{h}$.

Figure \ref{fig:SHDG MHDG CG} depicts the local/global degrees of freedom for the standard element HDG, macroelement HDG and CG methods in a sixteen-element mesh. The three schemes differ from each other not only in the degrees of freedom of the approximate $\left(\mathbf{q}_{h}, {u}_{h} \right)$, but also trace $\widehat{u}_{h}$.

The resulting method has a characteristic of the HDG method on the boundary faces of $\mathcal{T}^{i}_{h}$ and a characteristic of the CG method on interior locally DOFs. We note that the macroelements HDG method enjoys advantages of both the HDG and the CG methods. First, macroelements HDG inherits the reduced
number of global and local degrees of freedom of HDG. In fact, thanks to the macroelements HDG approach generates a global matrix system for the approximation on the boundaries of $\mathcal{T}^{i}_{h}$ that reduced rank of global matrix system in HDG, and has significantly smaller bandwidth than CG. As a result, the globally/locally coupled unknowns of the macroelements HDG method are even less than the HDG method, and is more efficient than both CG and HDG. Second, the macroelements HDG scheme enforces the boundary conditions as strongly as the HDG method, thus retaining the boundary condition robustness of HDG. These features make the macroelements HDG method an excellent alternative to the HDG and CG methods.

\subsubsection{Finite element spaces on global variable}

\begin{figure}
    \centering
     \subfloat[\centering HDG scheme.]{{\includegraphics[width=0.33\textwidth]{tikz/HDGTrace.pdf} }}%
     \subfloat[\centering CG-HDG scheme.]{{\includegraphics[width=0.33\textwidth]{tikz/CGDGTrace.pdf} }}%
     \subfloat[\centering Ptch-CG scheme.]{{\includegraphics[width=0.33\textwidth]{tikz/PTCHCGTrace.pdf} }}\\ %% 
    \caption{Illustration of the degrees of freedom for the standard HDG, CG-HDG and Ptch-CG scheme for the trace variable.}%
    \label{fig:HDG CG PTCH}%
\end{figure}

Same the above section, we have three options to introduce the finite space on traces variables. In the first case, CG-HDG scheme, trace variables are identical to variables located on elements boundaries which are shared by patches boundaries \cite{{vymazal2018combined}}, see Figure \ref{fig:HDG CG PTCH} (b). In the second case, Ptch-CG, we introduce variable based on patches boundaries, see Figure \ref{fig:HDG CG PTCH}(c). The CG-HDG method, on the other hand, introduces an additional hybrid variable on each patches, thus requiring more memory storage. In principle, when using Ptch-CG method on triangles in 2D and tetrahedral in 3D the number of non-zero blocks in each row, except for boundary elements, is 5 in 2D and 7 in 3D. We note that this pattern is common to the standard HDG scheme. However, the CG-HDG scheme is noncompactnes and therefore has a larger number of non-zero blocks with large $N_{i}^{Elm}$.

\begin{table}
\caption{Expressions for some parameters on an i-dimensional for meshes of Figure \ref{fig:Mesh2d and 3d}.}
\centering
\begin{tabular}{cccccc}\toprule
			& $ N^{ptch}$ 		 		&$N^{Elm}$ 		&$N^{face}$     &$N_{B.C}^{\Gamma_{i}}$ 	&$\text{dof}^{local}_{i}$\\[6pt]\hline
 $d = 2$ 	&$2\left( N_{e}\right)^{2}$  &$2\left( N_{e} N_{e}^{1D}\right)^{2}$	&3   &$4 \left(N_{e}\right)$ &$\left(N_{e}^{1D}  \rho+  1 \right)\left(N_{e}^{1D} \rho+  2 \right)/2 $\\ [6pt]
 $d = 3$ 	&$6\left( N_{e}\right)^{3}$ 	&$6\left( N_{e} N_{e}^{1D}\right)^{3}$ 	&4   &$6\left(2 N_{e}^{2}\right)$ &$\left(N_{e}^{1D}  \rho+  1 \right)\left(N_{e}^{1D} \rho+  2 \right)\left(N_{e}^{1D} \rho+  3 \right)/6 $ \\\bottomrule
 \hline
\end{tabular}
\label{Tab:Number patch and ...}%
\end{table}

The cases of triangular and tetrahedral meshes with polynomials of degree $\rho$ are considered. We assume that if $N_{e}$ is the number of patches in one direction, the number of triangles in 2D is $2N_{e}^{2}$ and the number of tetrahedra in 3D is $6N_{e}^{3}$, each patch consisting of $N_{i}^{Elm} = \left( N_{e}^{1D}\right)^{d} $, see Figure \ref{fig:Mesh2d and 3d}. These assumptions are reasonable for large and well shaped meshes, and are consistent with those in \cite{{vymazal2018combined, huerta2013efficiency}}. Table \ref{Tab:Number patch and ...} determines the values of $ N^{ptch}$, $N^{Elm}$, $N_{B.C}^{\Gamma_{i}}$, and, consequently, $\text{dof}^{local}_{i}$ for meshes.




\begin{equation}\label{TFlp}
N^{\Gamma_{i}}   =
	\begin{cases}
	\dfrac{N^{ptch} N^{face} -N_{B.C}^{\Gamma_{i}}}{2}    \quad\quad \; & \text{Ptch-CG}, \\[8pt]
	\dfrac{\left(N^{ptch} N^{face} -N_{B.C}^{\Gamma_{i}}\right)N_{e}^{1D}}{2}    \quad\quad  \; & \text{CG-HDG},\\[8pt]
	\dfrac{N^{Elm} N^{face} -N_{B.C}^{\Gamma_{i}}N_{e}^{1D}}{2}    \quad\quad \; & \text{HDG}.\\[8pt]
\end{cases} 
\end{equation}












In order quantify the matrix storage requirements for the three schemes, we consider the number of nonzero of global matrix entries. The total number of nonzeros is then 
\begin{equation}
M_{NON} = N^{\Gamma_{i}} \cdot N^{Blc} \cdot \left( dof^{\Gamma_{i}}\right) ^{2}.
\end{equation}
Where $N^{\Gamma_{i}}$ is the number of trace variables and $N^{Blc}$ is the number of non-zero blocks in each row with rank $dof^{\Gamma_{i}}$, the number of degrees of freedom per trace variable. Many of the key operations listed in Table \ref{Tab:operation Global}.


 \begin{table}
\caption{Number of operation for triangles/tetrahedral patch in 2D/3D for the Ptch-CG, CG-HDG, and HDG schemes, polynomial order $p$ and varying in $N_{e}^{1D}$.} 
\centering
\begin{tabular}{lllll}\toprule
  &Scheme        & $N^{\Gamma_{i}}$  & $N^{Blc}$ 	& $dof^{\Gamma_{i}}$   \\\midrule           
\multirow{3}{*}{$2D$}
&Ptch-CG  	&$ 3\left( N_{e}\right) ^{2} - 2N_{e}$	 &$5$		&$\left(N_{e}^{1D} \rho+  1 \right) $	\\[6pt]
&CG-HDG  	&$ \left( 3\left( N_{e}\right) ^{2} -2N_{e}\right)  N_{e}^{1D} $ 	&$5N_{e}^{1D}$ &$\left(\rho+  1 \right) $\\[6pt]
&HDG  	    	&$ 3\left( N_{e} N_{e}^{1D}\right) ^{2} -2N_{e} N_{e}^{1D} $	&$5$		&$\left(\rho+  1 \right) $		\\\midrule
\multirow{3}{*}{$3D$}
&Ptch-CG 	&$ 12 \left( N_{e}\right) ^{3} - 6 \left( N_{e}\right) ^{2}$	&$7$		&$\left(N_{e}^{1D}  \rho+  1 \right)\left(N_{e}^{1D} \rho+  2 \right)/2 $	\\[6pt]
&CG-HDG  	&$\left( 12 \left( N_{e}\right) ^{3} - 6 \left( N_{e}\right) ^{2}\right) \left(N_{e}^{1D}\right) ^{2}$	&$7 \left( N_{e}^{1D}\right) ^{2}$		&$\left(\rho+  1 \right) \left(\rho+  2 \right)/2 $\\[6pt]
&HDG  		&$12 \left( N_{e} N_{e}^{1D}\right) ^{3} - 6 \left( N_{e} N_{e}^{1D}\right) ^{2} $	&$7$		&$\left(\rho+  1 \right) \left(\rho+  2 \right)/2 $\\\bottomrule
\end{tabular}
\label{Tab:operation Global}%
\end{table}

 \begin{table}
\caption{Nonzeros of global matrix requirements for two triangles patches in 2D for the Ptch-CG, CG-HDG, and HDG schemes, polynomial order $p$ and varying in $N_{e}^{1D}$.} 
\centering
\begin{tabular}{llccccc}\toprule
  &Scheme        & $p = 1$   & $p = 2$  & $p = 3$ 	& $p = 4$   & $p = 5$  \\\midrule           
\multirow{3}{*}{$N_{e}^{1D} =2$}
&Ptch-CG  	&4.50E+01	&1.25E+02	&2.45E+02	&4.05E+02	&9.11E+04		\\[6pt]
&CG-HDG  	&8.00E+01	&1.80E+02	&3.20E+02	&5.00E+02	&2.27E+05    	\\[6pt]
&HDG  	    &1.60E+02	&3.60E+02	&6.40E+02	&1.00E+03	&1.32E+05		\\\midrule
\multirow{3}{*}{$N_{e}^{1D} =4$}
&Ptch-CG  	&1.25E+02	&4.05E+02	&8.45E+02	&1.45E+03	&2.21E+03		\\[6pt]
&CG-HDG  	&3.20E+02	&7.20E+02	&1.28E+03	&2.00E+03	&2.88E+03		\\[6pt]
&HDG  		&8.00E+02	&1.80E+03	&3.20E+03	&5.00E+03	&7.20E+03		\\\bottomrule
\end{tabular}
\label{Tab:nonzeros in 2D}%
\end{table}


 \begin{table}
\caption{Nonzeros of global matrix requirements for two tetrahedral patches in 3D for the Ptch-CG, CG-HDG, and HDG schemes, polynomial order $p$ and varying in $N_{e}^{1D}$.} 
\centering
\begin{tabular}{llccccc}\toprule
  &Scheme        & $p = 1$   & $p = 2$  & $p = 3$ 	& $p = 4$   & $p = 5$  \\\midrule           
\multirow{3}{*}{$N_{e}^{1D} =2$}
&Ptch-CG  	&1.62E+03	&1.01E+04	&3.53E+04	&9.11E+04	&1.96E+05		\\[6pt]
&CG-HDG  	&9.07E+03	&3.63E+04	&1.01E+05	&2.27E+05	&4.45E+05		\\[6pt]
&HDG  	    &5.29E+03	&2.12E+04	&5.88E+04	&1.32E+05	&2.59E+05		\\\midrule
\multirow{3}{*}{$N_{e}^{1D} =4$}
&Ptch-CG  	&1.01E+04	&9.11E+04	&3.73E+05	&1.05E+06	&2.40E+06		\\[6pt]
&CG-HDG  	&1.45E+05	&5.81E+05	&1.61E+06	&3.63E+06	&7.11E+06		\\[6pt]
&HDG  		&4.54E+04	&1.81E+05	&5.04E+05	&1.13E+06	&2.22E+06		\\\bottomrule
\end{tabular}
\label{Tab:nonzeros in 3D}%
\end{table}

The memory requirements for $N_{e} = 1$, $N_{e}^{1D} = 2,4$ and $\rho = 1,..., 5$ are shown in Table \ref{Tab:nonzeros in 2D} and \ref{Tab:nonzeros in 3D}.
We note that the Ptch-CG method has the lowest memory requirements. For instance, in three dimensions with polynomials of degree $\rho = 3$ and $N_{e}^{1D} =4$, the additional storage requirements of the HDG and CG-HDG methods are $35\%$ and $331\%$, respectively


\begin{equation}\label{TFlp}
M_{local}^{\text{Std}} =
	\begin{cases}
N^{Elm} \cdot \mathcal{O}\left(\left( \left(\rho+  1 \right)\left(\rho+  2 \right)/2\right) ^{3} \right) =    2\left( N_{e} N_{e}^{1D}\right)^{2} \cdot \mathcal{O}\left(\rho ^{6} \right) \quad \; &d = 2, \\[8pt]
N^{Elm} \cdot \mathcal{O}\left(\left(\left(\rho+  1 \right) \left(\rho+  2 \right)\left(\rho+  3 \right)/6\right) ^{3} \right) = 6\left( N_{e} N_{e}^{1D}\right)^{3} \cdot \mathcal{O}\left(\rho ^{9} \right) \quad \; &d = 3, \\[8pt]
\end{cases} 
\end{equation}


\begin{equation}\label{TFlp}
M_{local}^{\text{Mcr}} =
	\begin{cases}
N^{Ptch} \cdot \mathcal{O}\left(\left(\text{dof}^{local}_{i}\right) ^{3} \right) =    2\left( N_{e}\right)^{2} \cdot \mathcal{O}\left(\left(N_{e}^{1D}\rho \right) ^{6} \right) \quad \; &d = 2, \\[8pt]
N^{Ptch} \cdot \mathcal{O}\left(\left(\text{dof}^{local}_{i}\right) ^{3} \right) = 6\left( N_{e}\right)^{3} \cdot \mathcal{O}\left(\left(N_{e}^{1D}\rho\right) ^{9} \right) \quad \; &d = 3, \\[8pt]
\end{cases} 
\end{equation}




\subsection{Macroelement discretization}\label{S331}

Each patch  is seen as a ’macroelement’, where the governing equation is discretized by continuous Galerkin solver, while they are coupled together as in HDG. This means that the hybrid variable is only defined on inter-partition boundaries. A macroelement solver with Dirichlet data prescribed by the hybrid variable can be obtained by eliminating the flux variable from the system and reverting back to primal form for the unknown. In other hands, the standard element HDG applied to a single element, $ K $, and macroelement HDG would be applied to the whole $ \mathcal{T}^{i}_{h} $. 
The macroelement HDG discretization of Equations (\ref{C22}) reads as follows: Find $\left(\mathbf{q}_{h}, {u}_{h} \right)\in \widetilde{\bm{\mathcal{Q}}^{p}_{h}} \times \widetilde{\mathcal{V}^{p}_{h}}$ such that for all $ \mathcal{T}^{i}_{h} \in \mathcal{T}_{h}$
\begin{equation}\label{C33}
 \begin{split}
&\left( \mathbf{q}_{h},\bm{w}\right) _{\mathcal{T}^{i}_{h}} + \left( {u}_{h},\nabla\cdot\bm{w}\right) _{\mathcal{T}^{i}_{h}} -\left\langle  \widehat{u}_{h} ,\bm{w}\cdot\bm{n}\right\rangle  _{\partial \mathcal{T}^{i}_{h}} &= 0,	\quad
&\forall \bm{w} \in \left( \mathcal{P}_{p}\left( K\right) \right) ^{d},\\
&\left( \mathbf{F}_{h}^{\text{adv}} + \mathbf{F}_{h}^{\text{diff}},\nabla v\right) _{\mathcal{T}^{i}_{h}} - 
\left\langle  \left( \widehat{\mathbf{F}}_{h}^{\text{adv}}+\widehat{\mathbf{F}}_{h}^{\text{diff}}\right) \cdot\bm{n},v \right\rangle  _{\partial \mathcal{T}^{i}_{h}} - \left( f,v\right) _{\mathcal{T}^{i}_{h}}&= 0, \quad
&\forall v \in \mathcal{P}_{p}\left( K\right) .  
\end{split} 
\end{equation}
By adding the contributions of Equations (\ref{C33}) over all the macroelements and enforcing the continuity of the normal component of the numerical flux, we arrive at the following problem:
\begin{subequations}\label{C36}
 \begin{align}
&\left( \mathbf{q}_{h},\bm{w}\right) _{\mathcal{T}_{h}} + \left( {u}_{h},\nabla\cdot\bm{w}\right) _{\mathcal{T}_{h}} - \left\langle \widehat{u}_{h} ,\bm{w}\cdot\bm{n}\right\rangle  _{\Gamma} &= 0,	\quad &\forall \bm{w} \in \widetilde{\bm{\mathcal{Q}}}^{p}_{h},\label{C36A}\\
&\left(\mathbf{F}_{h}^{\text{adv}} + \mathbf{F}_{h}^{\text{diff}},\nabla v\right) _{\mathcal{T}_{h}} - 
\left\langle  \left( \widehat{\mathbf{F}}_{h}^{\text{adv}}+\widehat{\mathbf{F}}_{h}^{\text{diff}}\right) \cdot\bm{n},v\right\rangle  _{\Gamma} - \left( f,v\right) _{\mathcal{T}_{h}}&= 0,	\quad &\forall v \in \widetilde{\mathcal{V}}^{p}_{h},\label{C36B} \\
&\left\langle  \left( \widehat{\mathbf{F}}_{h}^{\text{adv}}+\widehat{\mathbf{F}}_{h}^{\text{diff}}\right) \cdot\bm{n},\mu\right\rangle  _{\Gamma\backslash\partial\Omega} 
 + \left\langle  \widehat{b}_{h},\mu\right\rangle  _{\partial\Omega}&= 0, \quad &\forall \mu \in \mathcal{M}^{p}_{h}. \label{C34C} 
\end{align}   
\end{subequations}
As before, we take the interior numerical fluxes of form
\begin{equation}\label{C37}
 \begin{split}
&\widehat{\mathbf{F}}_{h}^{\text{adv}}\cdot\bm{n} = 
\mathbf{c}\widehat{u}_{h}\cdot\bm{n}+
\tau_{\text{adv}}(u_{h}-\widehat{u}_{h}) \;\;\;\; &&on \; \Gamma,\\
&\widehat{\mathbf{F}}_{h}^{\text{diff}}\cdot\bm{n} = 
-\kappa\mathbf{q}_{h}\cdot\bm{n} +
\tau_{\text{diff}}(u_{h}-\widehat{u}_{h}) \;\;\;\; &&on \; \Gamma.
\end{split}   
\end{equation} 
Based on Equations (\ref{C37}) and (\ref{C35}), we defined numerical fluxes on interface of macroelements, $\Gamma_{i}$, while  is introduced on the boundary of elements by standard elements discretization. Like in the HDG method, the stabilization matrix is usually given by the contribution of $\tau_{\text{adv}}$ and $\tau_{\text{diff}}$ stabilization terms.

\subsubsection{Streamline upwind Petrov–Galerkin}

\begin{figure}
    \centering
    \subfloat[\centering Macroelement HDG with SUPG]{{\includegraphics[width=0.5\textwidth]{tikz/MHDGwithsupg.pdf} }}%
    \subfloat[\centering Macroelement HDG]{{\includegraphics[width=0.5\textwidth]{tikz/MHDGwithoutsupg.pdf} }}%
    \caption{Comparison between macroelement with/without stabilized (SUPG) approximations for advection dominated limits, $ \kappa=10^{-5} $.}%
    \label{fig:supg}%
\end{figure}

In literature consistent Petrov Galerkin formulations that are used to obtain non-oscillatory solutions 
for convection dominated problems are known as stabilized formulations. The general form of a consistent stabilization technique is \cite{donea2003finite} 

\begin{equation}\label{C39}
 \begin{split}
&\left( \mathbf{F}_{h}^{\text{adv}}\left( u_{h}\right)  + \mathbf{F}_{h}^{\text{diff}}\left( u_{h},\mathbf{q}_{h}\right) ,\nabla v)_{\mathcal{T}_{h}} - 
\left\langle  \right( \widehat{\mathbf{F}}_{h}^{\text{adv}}+\widehat{\mathbf{F}}_{h}^{\text{diff}})\cdot\bm{n},v \right\rangle  _{\Gamma} - \left( f,v\right) _{\mathcal{T}_{h}} \\
&+ \underbrace{\sum_{e}\int_{\Omega^{e}} \mathcal{P}\left(v\right) \tau_{\text{SUPG}}\mathcal{R}\left( u_{h}\right) }_\text{Stabilization term}= 0,
\end{split}
\end{equation}
where $\mathcal{P}\left(v\right) $ is some operator applied to the test functions, $\mathcal{R}\left( u_{h}\right) $ is the residual of the equation, and $\tau_{\text{SUPG}}$ is the stabilization parameter. In the SUPG method, 

\begin{equation}\label{C40}
 \begin{split}
& \mathcal{P}\left( v\right)   = \mat c \cdot \nabla v,\\
& \mathcal{R}\left( u_{h}\right)   = \nabla \cdot\left( \mat{F}^{\text{adv}}+\mat{F}^{\text{diff}} \right) - f,\\
& \tau_{\text{SUPG}}  =\dfrac{h}{2 \parallel \mat c \parallel} \:\left( \text{coth} \,\text{Pe} + \dfrac{1}{\text{Pe}} \right) .\\
\end{split}
\end{equation}
where $\text{Pe}$ is the mesh Péclet number, defined as $\text{Pe} =  \parallel \mat c \parallel h / \kappa$ and  $\parallel \mat c \parallel$ is the modulus of the convective velocity.

We compare the results obtained with HDG method on macroelement with/without SUPG formulations, Figure \ref{fig:supg}. As can be noticed, the macroelement with SUPG formulation provides a somewhat more steep slope in the jump while there appears to be slightly high oscillations. We consider an example of convection–diffusion skew to the mesh, proposed in Figure \ref{fig:test case}, the diffusivity coefficient is taken to be $\kappa = 10^{-5}$, number of elements $N^{Elm} = 3200$, and number of patches $N^{ptch}=50$. 

\subsection{Comparison of HDG on standard and macroelement schemes}
\begin{figure}
    \centering
    \subfloat[\centering Two dimension]{{\includegraphics[width=0.49\textwidth]{tikz/Mesh2d.pdf} }}%
    \subfloat[\centering Three dimension]{{\includegraphics[width=0.51\textwidth]{tikz/Mesh3d.pdf} }} %
    \caption{Plot of elements (back line) and patches pattern (blue line) used advection-diffusion 2D and 3D problems.}%
    \label{fig:Mesh2d and 3d}%
\end{figure}

For comparison to different HDG schemes, we consider the test case presented in Section (\ref{sec:Governing equations and test case description}) to demonstrate the optimal accuracy of the proposed schemes. The example presents as validation in the weakly advection-dominated regime, $ \kappa = 0.4 $. The source term $ f $ and Dirichlet boundary condition $ g_{D} $ are given by Equation (\ref{C24}). The cases of $ N^{Elm}=50 $ triangular (2D) and $ N^{Elm}=384 $ tetrahedral (3D) meshes, giving uniform element sizes of $ h$,  with elements per patch $ N_{i}^{Elm} =4$ (2D) and $ N_{i}^{Elm} =8$ (3D) are considered in Figure \ref{fig:Mesh2d and 3d}. We fixed number of elements per patch and consider solutions of polynomial degree $ p $ represented using a nodal basis within each element. In Figure \ref{fig:rate2d and 3d}, we present the error and convergence rate in $ L^{2}- $norm for the both schemes. We observe that in both cases the approximate solution converges optimally with order $ p+1 $ for $ p=1-4 $.

\begin{figure}
    \centering
    \subfloat[\centering Standard element, 2D]{{\includegraphics[width=0.5\textwidth]{tikz/Element-rate.pdf} }}%
    \subfloat[\centering Macroelement, 2D]{{\includegraphics[width=0.5\textwidth]{tikz/Patch-rate.pdf} }}\\ %
    \subfloat[\centering Standard element, 3D]{{\includegraphics[width=0.5\textwidth]{tikz/Element-rate3D.pdf} }}%
    \subfloat[\centering Macroelement, 3D]{{\includegraphics[width=0.5\textwidth]{tikz/Patch-rate3D.pdf} }}%
    \caption{Convergence rates for HDG on standard elements and macroelement with (SUPG) approximations in the weakly advection-dominated regime on 2D and 3D problem under uniform refinement.}%
    \label{fig:rate2d and 3d}%
\end{figure}







==> sections/old/Numerical_and_performance_results.tex <==
\section{ Numerical and performance results \label{sec: Numerical and performance results}}


In the following sections, we present numerical results that demonstrate several important features of the macroelement HDG solver and its performance when applied to a variety of test cases, elements size, patch size, polynomial order and number processes. We consider three-dimensional problems for linear advection-diffusion equations. 
xIn this study, we mainly use PETSc \cite{{balay2019petsc}} library as the solver of this linear system. In practice, we consider the provided GMRES iterative solver pre-conditioned with an algebraic additive Schwarz domain decomposition with one-levels of overlap, ASDD(1). Moreover, each one of the overlapped sub-problems is approximated with an incomplete LU factorization with zero fill-in, ILU(0). ASDD(1)/ILU(0) provides the best balance between communication cost and number of GMRES iterations for a variety of flow regimes, accuracy orders and number of processors \cite{{roca2013scalable}}.


\subsection{3D Linear advection-diffusion equations}\label{S5.1}

In this example, we provide a test case for the three-dimensional advection-diffusion equations. We consider the cube $[-0.5, 0.5]^{3}$ in $\mathbf{c}=(1,1,1)$, see Figure \ref{fig:Test case Brick3D}(a). The solution and refinement of level 5 are shown in Figure \ref{fig:Test case Brick3D}.

 \begin{figure}
    \centering
     \subfloat[\centering Test case.]{{\includegraphics[width=0.5\textwidth]{tikz/Testcase3D.pdf} }}%
     \subfloat[\centering Refinement of level 4.]{{\includegraphics[width=0.5\textwidth]{tikz/Brickref4.pdf} }}\\ %
     \subfloat[\centering Refinement of level 5 and Solution.]{{\includegraphics[width=0.5\textwidth]{tikz/BrickSref5.pdf} }}%
     \subfloat[\centering Volume slice.]{{\includegraphics[width=0.5\textwidth]{tikz/BrickSlices.pdf} }}
    \caption{Sequence of macroelement pattern and corresponding solution generated by a refinement scheme for advection–diffusion 3D problem.}%
    \label{fig:Test case Brick3D}%
\end{figure}


\subsubsection{Parallel scalability}\label{S5.1.1}
 The parallel behavior of both the solvers is shown in Figure \ref{fig:Scaling Element 3D} by a strong scaling experiment in same element number, using $N^{Elm}=124,096$ with $p=2$, but different patch size. Execution the local, global computations time(s) and number of iterations of the linear solver experiment presented in Table \ref{Tab:Brick3D,p2,scaling}, as well number of local and global unknowns for this test case can be seen in Table \ref{Tab:3D,patch size}. Namely, good performance of the number of iteration is seen over a range of $Cores$ and $N_{i}^{Elm}$ for the macroelement HDG method. 
 
 
While iteration counts may provide an estimate of how well the macroelement HDG method perform relative the patch size, the most important metric for evaluating the
performance of the solver is the total time taken. The $N_{i}^{Elm} =8$ and $N_{i}^{Elm} =64$ perform similarly in terms of the number of iterations solver and global time. However, the $N_{i}^{Elm} =64$ is slightly more expensive in terms of local time, thus the $N_{i}^{Elm} = 8$ performs the best in terms of total time for each number processor. The strong scaling of each $N_{i}^{Elm}$ for the local solver is shown in Figure \ref{fig:Scaling Element 3D}(a). The performance of the strong scaling of global solver improves with increasing patch size, see Figure \ref{fig:Scaling Element 3D}(b).  



 \begin{table}
\caption{Execution the local, global computations time(s) and number of iterations of the GMRES linear solver with an ASDD(1)/ILU(0) preconditioner in the advection–diffusion 3D problem, using $N^{Elm}=124,096$ with $p=2$, and varying in $N_{i}^{Elm}$.} 
\centering
\begin{tabular}{lcclcclccl}\toprule
& \multicolumn{3}{c}{$N_{i}^{Elm} = 1$} & \multicolumn{3}{c}{$N_{i}^{Elm} =8$}& \multicolumn{3}{c}{$N_{i}^{Elm} =64$}
\\\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
          & Local   & Global  & Iter 	& Local   & Global  & Iter 		& Local   & Global  & Iter\\\midrule           
 $Cores = 32$  			&2.24		&43.74	&649		&14.25		&1.88		&36	&83.90	&3.19		&32\\
 $Cores = 64$  			&1.12		&25.07	&646		&7.23		&1.10		&37	&47.61	&1.90		&33\\
 $Cores = 96$  			&0.75		&20.03	&657		&4.84		&0.85		&37	&30.99	&1.27		&33\\
 $Cores = 128$  			&0.56		&17.31	&656		&3.63		&0.76		&37	&22.18	&0.99		&33\\
 $Cores = 160$  			&0.44		&16.36	&660		&2.85		&0.63		&37	&16.80	&0.80		&34\\
 $Cores = 192$  			&0.37		&15.56	&652		&2.34		&0.67		&38	&13.63	&0.70		&35\\
 $Cores = 224$			&0.31		&15.25	&656		&1.98		&0.61		&37	&11.06	&0.62		&35\\\bottomrule
\end{tabular}
\label{Tab:Brick3D,p2,scaling}%
\end{table}

\begin{table}
\caption{Number of local and global unknowns and local unknowns per patch in the advection–diffusion 3D problem, using $N^{Elm}=124,096$ with $p=2$, and varying in $N_{i}^{Elm}$.} 
\centering
\begin{tabular}{llll} 
 \hline
 Size/Number 				& $N_{i}^{Elm} =1$ 		 &$N_{i}^{Elm} =8$ 		&$N_{i}^{Elm} =64$      \\\hline
 $\text{dof}^{local}$ 		&4,963,840  			 		    &2,171,680 					&1,279,740  \\ 
 $\text{dof}^{global}$ 	    &1,517,376 	 	 	 			&483,000 			    		&187,740    \\
 $N^{ptch}$ 					&124,096  		 	 			&15,512  					&1,939 		\\
 $\text{dof}^{local}_{i}$ 	&40  		 	 			 	&140 						&660  	    \\
 \hline
\end{tabular}
\label{Tab:3D,patch size}%
\end{table}


 \begin{figure}
    \centering
     \subfloat[\centering Scaling of local solver.]{{\includegraphics[width=0.5\textwidth]{tikz/LocalElm3D.pdf} }}%
     \subfloat[\centering Scaling of global solver.]{{\includegraphics[width=0.5\textwidth]{tikz/GlobalElm3D.pdf} }}
    \caption{Strong scaling of advection–diffusion 3D problem, using $N^{Elm}=124,096$ with $p=2$, and varying in $N_{i}^{Elm}$.}%
    \label{fig:Scaling Element 3D}%
\end{figure}



In Tables \ref{Tab:p1,Ptch cte, size} and \ref{Tab:3D, order size}, the local and global computations time(s), the iteration counts, number of local and global unknowns, and the corresponding number processor, are reported depending on varying in $p$ for $N_{i}^{Elm} =8$ cases. Also, the strong scaling of varying in $p$ for the $N^{Elm} = 45,568$ is shown in Figure \ref{fig:Scaling p}. The speedup quoted on the vertical axis is relative to the time taken on a single 32-processor node. At high polynomial order we clearly see that both local and global solver scale well.

 \begin{table}
\caption{Execution the local, global computations time(s) and number of iterations of the GMRES linear solver with an ASDD(1)/ILU(0) preconditioner in the advection–diffusion 3D problem, using $N^{ptch}=5,696$, $N^{Elm} = 45,568$ with $N_{i}^{Elm} =8$, and varying in $p$.} 
\centering
\begin{tabular}{lcclcclccl}\toprule
& \multicolumn{3}{c}{$p =2$} & \multicolumn{3}{c}{$p =3$}& \multicolumn{3}{c}{$p =4$}
\\\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
          & Local   & Global  & Iter 	& Local   & Global  & Iter 		& Local   & Global  & Iter\\\midrule           
 $Cores = 32$  	&5.16		&0.76		&36		&36.79		&2.80		&40	&216.20	&9.03		&44\\
 $Cores = 64$   &2.68		&0.55		&37		&18.52		&2.24		&40	&111.65	&5.66		&45\\
 $Cores = 96$  	&1.77		&0.41		&38		&12.38		&1.24		&40	&74.25	&4.34		&47\\
 $Cores = 128$	&1.35		&0.47		&37		&9.20		&1.05		&41	&55.10	&3.05		&46\\
 $Cores = 160$	&1.03		&0.43		&38		&7.30		&0.94		&41	&42.46	&2.93		&46\\
 $Cores = 192$	&0.86		&0.41		&39		&5.99		&0.82		&41	&35.29	&2.21		&48\\
 $Cores = 224$	&0.73		&0.39		&38		&5.17		&1.14		&42	&29.72	&1.93		&47\\\bottomrule
\end{tabular}
\label{Tab:p1,Ptch cte, size}%
\end{table}

\begin{table}
\caption{Number of local and global unknowns and local unknowns per patch in the advection–diffusion 3D problem, using $N^{ptch}=5,696$, $N^{Elm} = 45,568$ with $N_{i}^{Elm} =8$, and varying in $p$.} 
\centering
\begin{tabular}{llll} 
 \hline
 Size/Number 				& $p =2$ 		 			&$p =3$ 							&$p =4$ \\\hline
 $\text{dof}^{local}$ 		&797,440   			 		 &1,913,856 	 					&3,759,360  	 \\
 $\text{dof}^{global}$ 	    &179,880 	 	 	 		 &335,776 			    			&539,640  	 \\
 $\text{dof}^{local}_{i}$ 	&140   		 	 			 &336							&660   		 \\
  \hline
\end{tabular}
\label{Tab:3D, order size}%
\end{table}

 \begin{figure}
    \centering
     \subfloat[\centering Scaling of local solver.]{{\includegraphics[width=0.5\textwidth]{tikz/localP.pdf} }}%
     \subfloat[\centering Scaling of global solver.]{{\includegraphics[width=0.5\textwidth]{tikz/globalP.pdf} }}
    \caption{Strong scaling of advection–diffusion 3D problem, using $N^{ptch}=2874$ with $N_{i}^{Elm} =8$, and varying in $p$.}%
    \label{fig:Scaling p}%
\end{figure}
 
\begin{table}
\caption{Number of local and global unknowns and local unknowns per patch in the advection–diffusion 3D problem, using $\text{dof}^{local}\simeq 1,300,000$ and $\text{dof}^{local}\simeq 11,000,000$ with $p=2$, and varying in $N_{i}^{Elm}$.} 
\centering
\begin{tabular}{lllllll}\toprule
& \multicolumn{3}{c}{$\text{dof}^{local}\simeq 1,300,000$} & \multicolumn{3}{c}{$\text{dof}^{local}\simeq 11,000,000$}
\\\cmidrule(lr){2-4}\cmidrule(lr){5-7}
          					& $N_{i}^{Elm} =1$ &$N_{i}^{Elm} =8$ &$N_{i}^{Elm} =64$ 	& $N_{i}^{Elm} =1$ &$N_{i}^{Elm} =8$ &$N_{i}^{Elm} =64$\\\midrule           
 $\text{dof}^{local}$ 		&1,387,560  		&1,395,380	&1,279,740  &11,100,480		&11,163,040		&10,237,920	\\ 
 $\text{dof}^{global}$ 	    &427,932 	 	&311,970 	&187,740   	&3376,800		&2,443,920		&1,449,000\\
 $N^{Elm}$ 					&34,689  		&79,736  	&124,096  	&277,512			&637,888			&992,768\\
 $N^{ptch}$ 					&34,689  		&9,967  		&1,939 		&277,512			&79,736			&15,512\\
 $\text{dof}^{local}_{i}$ 	&40  		 	&140 		&660  		&40  		 	&140 			&660	\\\bottomrule
\end{tabular}
\label{Tab:DOF same size}%
\end{table}



   \begin{table}
\caption{Execution the local, global computations time(s) and number of iterations of the GMRES linear solver with an ASDD(1)/ILU(0) preconditioner in the advection–diffusion 3D problem, using $Cores = 224$ with $p = 2$, and varying in $N^{Elm}$ and $\text{dof}^{local}$.} 
\centering
\begin{tabular}{lcclcclccl}\toprule
& \multicolumn{3}{c}{$N_{i}^{Elm} = 1$} & \multicolumn{3}{c}{$N_{i}^{Elm} =8$}& \multicolumn{3}{c}{$N_{i}^{Elm} =64$}
\\\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
          									& Local   & Global  & Iter 	& Local   & Global  & Iter 		& Local   & Global  & Iter\\\midrule           
 $\text{dof}^{local}\simeq 1,300,000$  		&0.09		&4.90		&351		&1.26		&0.57		&39		&11.13	&0.64		&35\\
 $\text{dof}^{local}\simeq 11,000,000$  		&0.59		&2.90		&1092	&6.12		&1.53		&40		&58.87	&3.00		&34\\\bottomrule
\end{tabular}
\label{Tab:DOF same time}%
\end{table}


 \begin{table}
\caption{Execution the local, global computations time(s) and number of iterations of the GMRES linear solver with an ASDD(1)/ILU(0) preconditioner in the advection–diffusion 3D problem, using $\text{dof}^{local}\simeq 1,300,000$ with $p=2$, and varying in $N_{i}^{Elm}$.} 
\centering
\begin{tabular}{lcclcclccl}\toprule
& \multicolumn{3}{c}{$N_{i}^{Elm} = 1$} & \multicolumn{3}{c}{$N_{i}^{Elm} =8$}& \multicolumn{3}{c}{$N_{i}^{Elm} =64$}
\\\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
          & Local   & Global  & Iter 	& Local   & Global  & Iter 		& Local   & Global  & Iter\\\midrule           
 $Cores = 32$  			&0.63		&7.37		&315		&9.21		&1.55		&37	&85.62	&3.12		&32\\
 $Cores = 64$  			&0.31		&4.32		&325		&4.65		&0.94		&38	&47.69	&1.86		&33\\
 $Cores = 96$  			&0.21		&4.73		&335		&3.10		&0.77		&38	&30.88	&1.27		&33\\
 $Cores = 128$			&0.16		&4.62		&338		&2.35		&0.68		&38	&22.07	&1.04		&33\\
 $Cores = 160$			&0.12		&5.16		&342		&1.83		&0.66		&39	&16.70	&0.83		&34\\
 $Cores = 192$			&0.10		&5.18		&348		&1.49		&0.71		&39	&13.45	&0.71		&35\\
 $Cores = 224$			&0.09		&4.90		&351		&1.26		&0.57		&39	&11.13	&0.64		&35\\
 \bottomrule
\end{tabular}
\label{Tab:DOF same time scaling}%
\end{table}

 \begin{figure}
    \centering
     \subfloat[\centering Scaling of local solver.]{{\includegraphics[width=0.5\textwidth]{tikz/localDOF.pdf} }}%
     \subfloat[\centering Scaling of global solver.]{{\includegraphics[width=0.5\textwidth]{tikz/globalDOF.pdf} }}
    \caption{Strong scaling of advection–diffusion 3D problem, using $\text{dof}^{local}\simeq 1,300,000$ with $p=2$, and varying in $N_{i}^{Elm}$.}%
    \label{fig:Scaling DOF}%
\end{figure}



\subsubsection{Comparison of patch size}

In this section we compare the runtime performance and the number of GMRES iterations of the standard HDG with
the macroelement HDG in $h$ refinements. We choose the polynomial order $p = 2$, using $Cores = 130$, and for different parametric elements size. We present the results in Table \ref{Tab:Element ref with p2} and \ref{Tab:Time of Element ref with p2}. 

In $N^{Elm} = 992,768$, the local and global of unknowns are 40 and 12 million for $N_{i}^{Elm} = 1$, respectively. For $N^{Elm} = 992,768$, the macroelement whit $N_{i}^{Elm} = 8$ results in total times close to 21 times faster than standard HDG discretization, $N_{i}^{Elm} = 1$. In the case of the standard HDG merhod, we observe an increase in the number of GMRES iterations required, similar to what was observed in Table \ref{Tab:DOF same time}. For the $N_{i}^{Elm} = 1$, the number of iterations required for the ASDD(1)/ILU(0) preconditioner increases with $N^{Elm}$ at a faster rate when compared with the $N_{i}^{Elm} =64$, suggesting that the global solver in large patch size is most effective for $h$ refinements.

\begin{table}
\caption{Number of local and global unknowns in the advection–diffusion 3D problem, using $Cores = 130$ with $p = 2$, and varying in $N^{Elm}$.} 
\centering
\begin{tabular}{lllllll}\toprule
& \multicolumn{2}{c}{$N_{i}^{Elm} = 1$} & \multicolumn{2}{c}{$N_{i}^{Elm} = 8$}& \multicolumn{2}{c}{$N_{i}^{Elm} = 64$}
\\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
   & $\text{dof}^{local}$   & $\text{dof}^{global}$ 	& $\text{dof}^{local}$   & $\text{dof}^{global}$  & $\text{dof}^{local}$ & $\text{dof}^{global}$ \\\midrule           
 $N^{Elm} = 45,504$  		&182,0160		&560,448			&796,320			&179,640			&469,260				&70,740\\
 $N^{Elm} = 124,096$  		&4,963,840		&1,517,376		&2,171,680		&483,000			&1,279,740			&187,740\\
 $N^{Elm} = 364,032$  		&14,561,280		&4,425,984		&6,370,560		&1,401,120		&3,754,080			&538,920\\
 $N^{Elm} = 992,768$  		&39,710,720		&12,026,112		&17,373,440		&3,793,440		&10,237,920			&1,449,000\\\bottomrule
\end{tabular}
\label{Tab:Element ref with p2}%
\end{table}

\begin{table}
\caption{Execution the local, global computations time(s) and number of iterations of the GMRES linear solver with an ASDD(1)/ILU(0) preconditioner in the advection–diffusion 3D problem, using $Cores = 130$ with $p = 2$, and varying in $N^{Elm}$.} 
\centering
\begin{tabular}{lcclcclccl}\toprule
& \multicolumn{3}{c}{$N_{i}^{Elm} = 1$} & \multicolumn{3}{c}{$N_{i}^{Elm} =8$}& \multicolumn{3}{c}{$N_{i}^{Elm} =64$}
\\\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
          & Local   & Global  & Iter 	& Local   & Global  & Iter 		& Local   & Global  & Iter\\\midrule           
 $N^{Elm} = 45,504$  		&0.15	&3.31	&512		&0.47	&0.42	&37	&2.23	&0.49	&34\\
 $N^{Elm} = 124,096$  		&0.40	&7.72	&677		&1.27	&0.94	&37	&6.37	&0.92	&34\\
 $N^{Elm} = 364,032$			&1.21	&42.13	&1265	&3.8	0	&1.81	&37	&19.12	&2.35	&34\\
 $N^{Elm} = 992,768$  		&3.27	&237.9	&2297	&10.61	&4.03	&38	&53.44	&6.16	&33\\\bottomrule
\end{tabular}
\label{Tab:Time of Element ref with p2}%
\end{table}




\subsection{Advection–diffusion in a rotating cylinder}

In the last example we solved advection–diffusion in a three-dimensional cylinder that rotates around z-axis with advective velocity $c_{x}=-sin(\theta)\omega$, $c_{y}=cos(\theta)\omega$ and constant axial velocity $c_{z}=1.0$, which results in a helical pattern of the concentration. Here, the inflow boundary $u=1.0$, outflow boundary condition $u = 0$ and slip wall in surface cylinder were assumed on the whole boundary, see Figure \ref{fig:Test case Cyl3D}(a). Also, we fixed angular velocity $\omega=1.8$ and source term $f = 0$. Based on this characteristics, the Péclet number of this problem is $Pe = 360$.

The geometry of the cylinder is described by a grid of $6\times20\times10$ elements in  $(r, \theta, z)$-directions, respectively. Then we solve the problem whit $p=2$ and use our refinement strategy based on the gradient-based error indicator, and solve the problem in the locally refined mesh again. We continue this approach for refinement level 2. These plots are shown in Figure \ref{fig:Test case Cyl3D}(c) with 25,196 and (d) with 63,682 macroelements for locally refinement level 1 and 2, respectively. The plots of the flow for the refinement patches level 2 are shown in Figure \ref{fig:Solution Cyl3D}. Furthermore, the locally refinement level 2 has successfully resolved the areas in the form of a helix which are improving resolution of the boundary and internal layers.

Several parameters have been varied to obtain the results. First, the code has been launched with different number of processors, that also correspond to the number of $N_{i}^{Elm}$. To this end, meshes with different interpolation degree, $p$, and number of elements, $N^{Elm}$, have been generated.


 \begin{figure}
    \centering
     \subfloat[\centering Test case.]{{\includegraphics[width=0.5\textwidth]{tikz/Cyl3D.pdf} }}%
     \subfloat[\centering Patch volume refinement.]{{\includegraphics[width=0.5\textwidth]{tikz/Cyl3DElm.pdf} }}\\ %
     \subfloat[\centering Refinement of level 1.]{{\includegraphics[width=0.5\textwidth]{tikz/Cyl3DRef1.pdf} }}%
     \subfloat[\centering Refinement of level 2.]{{\includegraphics[width=0.5\textwidth]{tikz/Cyl3DRef2.pdf} }}
    \caption{Sequence of patches pattern generated by a refinement scheme for advection–diffusion 3D problem in a rotating cylinder.}%
    \label{fig:Test case Cyl3D}%
\end{figure}


 \begin{figure}
    \centering
     \subfloat[\centering Corresponding solution.]{{\includegraphics[width=0.5\textwidth]{tikz/Cyl3DSolution.pdf} }}%
     \subfloat[\centering Solution of mesh refinement.]{{\includegraphics[width=0.5\textwidth]{tikz/Cyl3DSolution2.pdf} }}
    \caption{Solution for the advection–diffusion 3D problem in a rotating cylinder.}%
    \label{fig:Solution Cyl3D}%
\end{figure}


\subsubsection{Parallel scalability}\label{S5.2.1}
 In this example, we want to check the execution computation time, strong scaling and degrees of freedom of local and global solver. In Table \ref{Tab:Cyl3D,dof size}, we have listed the the number of local and global unknowns for a mesh with 254,208 elements of order 2 using different number of patch size, $N_{i}^{Elm}$. This mesh
has around 10.2 million local unknowns $({u}_{h})$ and 3.1 million global unknowns $(\widehat{u}_{h})$ in standard HDG discretization, whereas the macroelement HDG discretization with $N_{i}^{Elm} =64$ requires only 2.6 and 0.4 million local and global unknowns, respectively. 
 
In Table \ref{Tab:Cyl3D,scaling} we have summarized the computation time for the local and global stages of different number of processors. The time balance between the two steps of patch size are also listed in this table. Again, we have used the ASDD(1)/ILU(0) preconditioner, and adjusted the relative tolerance of the global solver to $10^{-12}$. These timing results are obtained using 32 cores per node in a supercomputer. This means we have decomposed our domain to maximum 224 sub-domains and used one core for each sub-domain for global solver.  As explained in the two dimensional problem, the local computation time is again perfectly scaled by increasing the number of active cores, see Figure \ref{fig:Scaling Element Cyl3D}(a).  However, the global solver does not scale very well. It seems that the larger bandwidth of the global
matrix corresponding to the high patch size, $N_{i}^{Elm} =64$, has been handled very well by the parallel preconditioner and the global solver, Figure \ref{fig:Scaling Element Cyl3D}(b).



 \begin{table}
\caption{Execution the local, global computations time(s) and number of iterations of the GMRES linear solver with an ASDD(1)/ILU(0) preconditioner for the advection–diffusion 3D problem in a rotating cylinder, using $N^{Elm}=254,208$ with $p=2$, and varying in $N_{i}^{Elm}$.} 
\centering
\begin{tabular}{lcclcclccl}\toprule
& \multicolumn{3}{c}{$N_{i}^{Elm} = 1$} & \multicolumn{3}{c}{$N_{i}^{Elm} =8$}& \multicolumn{3}{c}{$N_{i}^{Elm} =64$}
\\\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
          & Local   & Global  & Iter 	& Local   & Global  & Iter 		& Local   & Global  & Iter\\\midrule           
 $Cores = 32$  			&4.7		&127.1		&902		&33.1		&4.6		&50		&201.8		&6.6		&50\\
 $Cores = 64$  			&2.3		&65.5		&879		&16.7		&2.6		&51		&110.3		&3.6		&51\\
 $Cores = 96$  			&1.5		&48.7		&875		&11.1		&1.8		&51		&71.7		&2.6		&52\\
 $Cores = 128$  			&1.2		&42.4		&893		&8.3			&1.5		&51		&52.5		&2.0		&49\\
 $Cores = 160$  			&0.9		&36.8		&892		&6.5			&1.3		&51		&40.3		&1.8		&55\\
 $Cores = 192$  			&0.7		&34.1		&901		&5.3			&1.2		&50		&32.5		&1.5		&52\\
 $Cores = 224$			&0.6		&30.3		&911		&4.5			&1.1		&51		&27.2		&1.2		&56\\\bottomrule
\end{tabular}
\label{Tab:Cyl3D,scaling}%
\end{table}

\begin{table}
\caption{Number of local and global unknowns and local unknowns per patch for the advection–diffusion 3D problem in a rotating cylinder, using $N^{Elm}=254,208$ with $p=2$, and varying in $N_{i}^{Elm}$.} 
\centering
\begin{tabular}{llll} 
 \hline
 Size/Number 				& $N_{i}^{Elm} =1$ 		 &$N_{i}^{Elm} =8$ 		&$N_{i}^{Elm} =64$ \\\hline
 $\text{dof}^{local}$ 		&10,168,320  			 		&4,448,640 			&2,621,520  \\ 
 $\text{dof}^{global}$ 	    &3,111,936 	 	 	 			&991,680 			&386,280  	\\
 $N^{ptch}$ 					&254,208  		 	 			&31,776  			&3,972 		\\
 $\text{dof}^{local}_{i}$ 	&40  		 	 			 	&140 				&660  		\\\hline
\end{tabular}
\label{Tab:Cyl3D,dof size}%
\end{table}




 \begin{figure}
    \centering
     \subfloat[\centering Scaling of local solver.]{{\includegraphics[width=0.5\textwidth]{tikz/LocalCyl3D.pdf} }}%
     \subfloat[\centering Scaling of global solver.]{{\includegraphics[width=0.5\textwidth]{tikz/GlobalCyl3D.pdf} }}
    \caption{Strong scaling of advection–diffusion 3D problem in a rotating cylinder, using $N^{Elm}=254,208$ with $p=2$, and varying in $N_{i}^{Elm}$.}%
    \label{fig:Scaling Element Cyl3D}%
\end{figure}



\subsubsection{Comparison of patch size}

The computation time for the most refined grid of different orders, i.e. 104,296 elements is presented in Table \ref{Tab:Cyl3D,order with patch size}. In this case with $p = 5$, we had around 23.4 and 14.9 million local unknowns, and 4.5 and 1.8 million global unknowns in $N_{i}^{Elm} = 1$ and $N_{i}^{Elm} = 8$, respectively. 
Also noticeable is that by increasing the  polynomial order the computational balance changes towards the local computation. 


To decide between macroelement size, it is also important to consider the execution time and iteration of global linear solver. 
To this end, Table \ref{Tab:Cyl3D,dof of elements with patch size} presents the number of local and global unknowns for the five elements size from 158,592 to 2,033,664. 
The results in Table \ref{Tab:Cyl3D,time of elements with patch size} show that global time and linear iteration that use a patch size with 1 are more expensive that the corresponding $N_{i}^{Elm} = 64$.

As with the previous test case, the number of iterations using the preconditioner grows with increasing number of elements. On the contrary, due to increasing patch size, the iteration of linear solver is weak scaling.




 \begin{table}
\caption{Number of local and global unknowns for the advection–diffusion 3D problem in a rotating cylinder, using $N^{Elm}=104,296$ with $Core =143$, and varying in $N_{i}^{Elm}$ of different orders, and the time spent for local and global computations time(s).} 
\centering
\begin{tabular}{ccccccccccc}\toprule
& \multicolumn{4}{c}{$N_{i}^{Elm} = 1$} & \multicolumn{4}{c}{$N_{i}^{Elm} =8$}
\\\cmidrule(lr){2-5}\cmidrule(lr){6-9}
          & $\text{dof}^{local}$   & $\text{dof}^{global}$  & Local   & Global  & $\text{dof}^{local}$   & $\text{dof}^{global}$  & Local   & Global\\\midrule           
 $p = 1$  			&1,668,736		&639,216			&0.11	&3.52	&521,480			&163,164			&0.04	&0.19\\
 $p = 2$  			&4,171,840		&1,278,432		&0.31	&6.80	&1,825,180		&407,910			&1.06	&0.88\\
 $p = 3$  			&8,343,680		&2,130,720		&1.16	&10.19	&4,380,432		&761,432			&9.86	&2.43\\
 $p = 4$  			&14,601,440		&3,196,080		&6.00	&18.24	&8,604,420		&1,223,730		&41.85	&7.67\\
 $p = 5$  			&23,362,304		&4,474,512		&32.06	&34.82	&14,914,328		&1,794,804		&175.83	&19.07\\\bottomrule
\end{tabular}
\label{Tab:Cyl3D,order with patch size}%
\end{table}







 \begin{table}
\caption{Number of local and global unknowns for the advection–diffusion 3D problem in a rotating cylinder, using $Core =143$ with $p=1$, and varying in $N_{i}^{Elm}$ of  $N^{Elm}$.} 
\centering
\begin{tabular}{lcccccc}\toprule
& \multicolumn{2}{c}{$N_{i}^{Elm} = 1$} & \multicolumn{2}{c}{$N_{i}^{Elm} =8$} & \multicolumn{2}{c}{$N_{i}^{Elm} = 64$}
\\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
          & $\text{dof}^{local}$   & $\text{dof}^{global}$  & $\text{dof}^{local}$   & $\text{dof}^{global}$  & $\text{dof}^{local}$   & $\text{dof}^{global}$\\\midrule           
 $N^{Elm}= 158,592$  			&2,537,472			&976,512				&792,960				&25,0368			&346,920			&82,140\\
 $N^{Elm}= 254,208$  			&4,067,328			&1,555,968			&1,271,040			&396,672			&556,080			&128,760\\
 $N^{Elm}= 596,224$  			&9,539,584			&3,627,264			&2,981,120			&919,296			&1,304,240		&295,080\\
 $N^{Elm}= 1,268,736$  			&20,299,776			&7,712,256			&6,343,680			&1,953,024		&2,775,360		&625,920\\
 $N^{Elm}= 2,033,664$  			&32,538,624			&12,324,864			&10,168,320			&3,111,936		&4,448,640		&991,680\\\bottomrule
\end{tabular}
\label{Tab:Cyl3D,dof of elements with patch size}%
\end{table}



 \begin{table}
\caption{Execution the local, global computations time(s) and number of iterations of the GMRES linear solver with an ASDD(1)/ILU(0) preconditioner  for the advection–diffusion 3D problem in a rotating cylinder, using $Core =143$ with $p=1$, and varying in $N_{i}^{Elm}$ of  $N^{Elm}$.} 
\centering
\begin{tabular}{lcclcclccl}\toprule
& \multicolumn{3}{c}{$N_{i}^{Elm} = 1$} & \multicolumn{3}{c}{$N_{i}^{Elm} =8$} & \multicolumn{3}{c}{$N_{i}^{Elm} = 64$}
\\\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
          						& Local   & Global  & Iter 	& Local   & Global  & Iter	& Local   & Global	& Iter\\\midrule           
 $N^{Elm}= 158,592$  			&0.16	&5.01	&967		&0.07	&0.16	&34	&0.21	&0.11	&23\\[5pt]
 $N^{Elm}= 254,208$  			&0.26	&9.54	&1128 	&0.11	&0.25	&35	&0.34	&0.22	&23\\[5pt]
 $N^{Elm}= 596,224$  			&0.61	&38.26	&1994	&0.25	&0.83	&33	&0.81	&0.62	&21\\[5pt]
 $N^{Elm}= 1,268,736$  			&1.23	&106.76	&2522	&0.53	&1.15	&32	&1.73	&0.71	&22\\[5pt]
 $N^{Elm}= 2,033,664$  			&2.16	&225.53	&2974	&0.89	&1.62	&31	&2.79 	&1.07   &23\\\bottomrule
\end{tabular}
\label{Tab:Cyl3D,time of elements with patch size}%
\end{table}




\subsection{Domain decomposed load balancing}


For domain decomposed applications it is always important to account for variable computational loads across processors and ensure that these loads are as even as possible. Failure to account for load imbalances can severely impact performance and limit the parallel strong/weak scaling. Improved load balancing results in significant improvements to runtime and speed up performance. To analyze the actual performance, the advection–diffusion 3D problem whit $N^{Elm} = 196,608$, $N_{i}^{Elm} = 8$ was run using $p=1$ and $2$. For a given cluster, the “load balancing performance factor” for each method is collected, which is calculated as being the ratio of the average time spent among processors to the maximum time spent of all processors. This ratio is a measure of the load balancing efficiency(LBF), and is defined as follows:
 \begin{align*}
    \text{Load	Balance	Efficiency} = \frac{\text{Avg. workload among procs}}{\text{Max. workload among procs}}.       
\end{align*}
A perfect balance scheme will result in a factor of 1.0, with less optimal load balancing schemes having ratios smaller than 1.0. There are different definitions in the literature, but mostly all based on average and maximum time spent. 
Figure \ref{fig:BL coarse order} depicts the breakdown of execution time for the case of a cluster with 8, 16 and 32 processors (1 node) for local and global solver. Based on these results, we see excellent load balancing in
terms of local and global computations. We also examine how the workload of each processor itself scales with the number of nodes, shown in Figure \ref{fig:BL fine order}. We obtain a varying LBF between 0.87 and 0.91 for different number of nodes. The efficiency remains above 0.87 and 0.91 in local/ global solver, even at 4 nodes and 128 processes, respectively.
\begin{figure}
    \centering
     \subfloat[\centering $Node = 1, LBF = 0.97$]{{\includegraphics[width=0.33\textwidth]{tikz/Uni8Local.pdf} }}%
     \subfloat[\centering $Node = 1, LBF = 0.98$]{{\includegraphics[width=0.33\textwidth]{tikz/Uni16Local.pdf} }}%
     \subfloat[\centering $Node = 1, LBF = 0.97$]{{\includegraphics[width=0.33\textwidth]{tikz/Uni32Local.pdf} }}\\ %%
     \subfloat[\centering $Node = 1, LBF = 0.92$]{{\includegraphics[width=0.33\textwidth]{tikz/Uni8Global.pdf} }}%
     \subfloat[\centering $Node = 1, LBF = 0.95$]{{\includegraphics[width=0.33\textwidth]{tikz/Uni16Global.pdf} }}%
     \subfloat[\centering $Node = 1, LBF = 0.97$]{{\includegraphics[width=0.33\textwidth]{tikz/Uni32Global.pdf} }} 
    \caption{Load balancing time of local (blue) and global solver (red) for advection–diffusion 3D problem whit $N^{Elm} = 196,608$, $N_{i}^{Elm} = 8$, $\text{dof}^{local} = 983,040$ and $\text{dof}^{global} = 608,256$ in $p=1$.}%
    \label{fig:BL coarse order}%
\end{figure}

\begin{figure}
    \centering
     \subfloat[\centering $Node = 1, LBF = 0.91$]{{\includegraphics[width=0.33\textwidth]{tikz/UniF32Local.pdf} }}%
     \subfloat[\centering $Node = 2, LBF = 0.90$]{{\includegraphics[width=0.33\textwidth]{tikz/UniF64Local.pdf} }}%
     \subfloat[\centering $Node = 4, LBF = 0.87$]{{\includegraphics[width=0.33\textwidth]{tikz/UniF128Local.pdf} }}\\ %%
     \subfloat[\centering $Node = 1, LBF = 0.87$]{{\includegraphics[width=0.33\textwidth]{tikz/UniF32Global.pdf} }}%
     \subfloat[\centering $Node = 2, LBF = 0.90$]{{\includegraphics[width=0.33\textwidth]{tikz/UniF64Global.pdf} }}%
     \subfloat[\centering $Node = 4, LBF = 0.91$]{{\includegraphics[width=0.33\textwidth]{tikz/UniF128Global.pdf} }} 
    \caption{Load balancing time of local (blue) and global solver (red) for advection–diffusion 3D problem whit $N^{Elm} = 196,608$, $N_{i}^{Elm} = 8$, $\text{dof}^{local} = 3,440,640$ and $\text{dof}^{global} = 1,216,512$ in $p=2$.}%
    \label{fig:BL fine order}%
\end{figure}

\begin{landscape} 

\end{landscape}


\subsection{Scaling with $h$ and $p$}


To study the convergence for iterative solver as function of the refining the elements ($h$-refinement) and the polynomial order ($p$-refinement), the problem is solved using the ASDD(0)/ILU(0) preconditioner, the $Core =32$, and the three diffusion values $\kappa=10^{-5}$, $\kappa=1$ and $\kappa=10^{5}$. The resulting numbers of iterations are shown in Table \ref{Tab:h and p iteration in 2D} and \ref{Tab:h and p iteration in 3D}. 

\begin{landscape}

 \begin{table}
\caption{Scaling of the convergence for the advection–diffusion 2D problem, as function of mesh size $h$, polynomial order $p$ and varying in $N_{i}^{Elm}$.} 
\centering
\begin{tabular}{llccccccccc}\toprule
&& \multicolumn{3}{c}{$N_{i}^{Elm} = 1$} & \multicolumn{3}{c}{$N_{i}^{Elm} =16$}& \multicolumn{3}{c}{$N_{i}^{Elm} =64$}
\\\cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}
  &        & $h = 0.03$   & $h = 0.02$  & $h = 0.01$ 	& $h = 0.03$   & $h = 0.02$  & $h = 0.01$ 		& $h = 0.03$   & $h = 0.02$  & $h = 0.01$\\\midrule           
\multirow{4}{*}{$\kappa=10^{-5}$}&$p = 2$&59		&181		&257		&18		&21		&22		&14		&15		&16\\
&$p = 3$  	&60			&212		&268		&19		&21		&22		&14		&15		&17\\
&$p = 4$  	&60			&262		&254		&19		&21		&22		&14		&16		&17\\
&$p = 5$  	&73			&285		&270		&20		&21		&22		&14		&16		&17\\\midrule
\multirow{4}{*}{$\kappa=1$}&$p = 2$  	&309		&569		&789		&90		&103		&150		&38		&72		&82\\
&$p = 3$  	&405			&659		&832		&87		&123		&164		&47		&80		&83\\
&$p = 4$  	&416			&685		&849		&95		&128		&167		&58		&82		&96\\
&$p = 5$  	&463			&742		&982		&95		&136		&168		&61		&84		&91\\\midrule
\multirow{4}{*}{$\kappa=10^{5}$}&$p = 2$ &287	&481		&806		&88		&112		&141		&38		&69		&79\\
&$p = 3$  	&346			&525		&830		&87		&121		&120		&46		&73		&82\\
&$p = 4$  	&361			&555		&880		&87		&123		&148		&54		&79		&94\\
&$p = 5$  	&364			&691		&943		&98		&127		&167		&55		&80		&88\\\bottomrule
\end{tabular}
\label{Tab:h and p iteration in 2D}%
\end{table}

 \begin{table}
\caption{Scaling of the convergence for the advection–diffusion 3D problem, as function of mesh size $h$, polynomial order $p$ and varying in $N_{i}^{Elm}$.} 
\centering
\begin{tabular}{llccccccccc}\toprule
&& \multicolumn{3}{c}{$N_{i}^{Elm} = 1$} & \multicolumn{3}{c}{$N_{i}^{Elm} =8$}& \multicolumn{3}{c}{$N_{i}^{Elm} =64$}
\\\cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}
  &        & $h = 0.07$   & $h = 0.05$  & $h = 0.03$ 	& $h = 0.07$   & $h = 0.05$  & $h = 0.03$ 		& $h = 0.07$   & $h = 0.05$  & $h = 0.03$\\\midrule           
\multirow{4}{*}{$\kappa=10^{-5}$}&$p = 2$  	&17			&18		&26		&11		&12		&16	&8	&9		&10\\
&$p = 3$  	&17		&18		&26		&11		&12			&16		&9		&9		&10\\
&$p = 4$  	&18		&19		&25		&12		&12			&16		&9		&9		&10\\
&$p = 5$  	&18		&18		&25		&12		&13			&16		&9		&9		&10\\\midrule
\multirow{4}{*}{$\kappa=1$}&$p = 2$  &127	&153			&267		&33		&33		&36		&29		&27		&31\\
&$p = 3$  	&148		&158		&292		&37		&35			&38		&33		&29		&34\\
&$p = 4$  	&160		&182		&319		&41		&40			&43		&36		&33		&38\\
&$p = 5$  	&163		&170		&353		&43		&42			&44		&38		&35		&40\\\midrule
\multirow{4}{*}{$\kappa=10^{5}$}&$p = 2$  	&130			&160		&268		&34		&33		&36		&30		&28		&32\\
&$p = 3$  	&148		&185		&313		&37		&36			&39		&33		&30		&35\\
&$p = 4$  	&162		&201		&349		&42		&40			&43		&37		&33		&39\\
&$p = 5$  	&172		&211		&368		&44		&42			&44		&40		&35		&41\\\bottomrule
\end{tabular}
\label{Tab:h and p iteration in 3D}%
\end{table}

\end{landscape}




==> sections/old/complexity.tex <==
\section{Computational complexity \label{sec:complexity}}

\subsection{Matrix problem}
We consider matrix problems of the following kind
\begin{align}
	\begin{bmatrix}
		A & B^T \\
		B & C
	\end{bmatrix}
	\begin{bmatrix}
		u  \\
		\hat{u} 
	\end{bmatrix} = 
	\begin{bmatrix}
		R_u  \\
		R_{\hat{u}} 
	\end{bmatrix}
\end{align}
where $u \in \mathbb{R}^z$ denote degrees of freedom associated with the discretization of a domain into discontinuous macro-elements and $\hat{u} \in \mathbb{R}^{\hat{z}}$ denotes a vector with degrees of freedom associated with the discretization of trace variables associated with the skeleton of the macro-element mesh. The matrices have a special block-structure due to the discontinuous nature of the approximation spaces and the coupling of patches by means of interface variables. In particular matrix $A$ is a block-diagonal matrix, each block associated with one macro-element. We assume all blockmatrices of $A$ are invertible.

Using the Schur complement the above matrix problem can be solved for $\hat{u}$ by condensing out the degrees of freedom $u$, which leads to
\begin{align}
	\left( C - B A^{-1} B^T \right) \hat{u} &= R_{\hat{u}} - B A^{-1} R_{\hat{u}} && (\text{Solve for interface dofs})	\label{eq:global_problem}	\\
	A \, u &= R_{u} - B^T \hat{u} && (\text{Solve for interior dofs})
	\label{eq:local_problem}
\end{align}
This may lead to an efficient solution methodology if the number of interface variables is much smaller than the original problem, that is, $\hat{z} << z$. 

Consider the following iterative solution approach to  \eqref{eq:global_problem}. First compute $f = R_{\hat{u}} - B A^{-1} R_{\hat{u}}$. Then solve $\left( C - B A^{-1} B^T \right) \hat{u} = f$ by an iterative solver that performs the matrix-vector product in the following steps:
\begin{enumerate}
	\item $x = B^T \hat{u}$
	\item $y = A^{-1} x$
	\item $\hat{v} = B y$
	\item $\hat{w} = C \hat{u} - \hat{v}$
\end{enumerate}
The block structure of the matrices $A$, $B$, and $C$ imply that the first three steps can be performed locally, for each macro-element in the mesh, separately. Step four can be performed locally, for each face in the mesh skeleton. In practice, the inverse of $A^{-1}$ is never computed. Instead, LU-factorizations of each block in $A$ are used.

\begin{example}
Consider the following two-macro-element mesh depicted in Figure \ref{fig:hdg}. We are interested in performing one matrix-vector multiplication in the iterative solution of \eqref{eq:global_problem}. The first three steps can be performed as follows
\begin{scriptsize}
\begin{align}
	\begin{bmatrix}
		x_{11} \\ x_{12} \\ x_{13} \\ \hline  x_{21} \\ x_{22} \\ x_{23}
	\end{bmatrix} = \underbrace{ 
	\begin{bmatrix}
		 * &  *  \\ * & * \\ * & * \\ \hline * & * \\ * & * \\ * & *
	\end{bmatrix}}_{B^T}
	\begin{bmatrix}
		\hat{u}_1  \\
		\hat{u}_2 
	\end{bmatrix},
&&
	\begin{bmatrix}
		y_{11} \\ y_{12} \\ y_{13} \\ \hline  y_{21} \\ y_{22} \\ y_{23}
	\end{bmatrix} = \underbrace{ 
	\begin{bmatrix}[c c c | c c c]
		 * & * & * &    &    &  \\ * & * & * &   &   &   \\ * & * & * &   &   &   \\ \hline 
			&		&		&		* &	*	& * \\	&		&		&		* &	*	& * \\ &		&		&		* &	*	& *
	\end{bmatrix}}_{A^{-1}}
	\begin{bmatrix}
		x_{11} \\ x_{12} \\ x_{13} \\ \hline  x_{21} \\ x_{22} \\ x_{23}
	\end{bmatrix},
&&
	\begin{bmatrix}
		\hat{v}_1  \\ \hat{v}_2
	\end{bmatrix} =  \underbrace{ 
	\begin{bmatrix}[c c c | c c c]
		 * & * & * &  *  & *  & * \\ * & * & * & * & * & * 
	\end{bmatrix}}_{B}
	\begin{bmatrix}
		y_{11} \\ y_{12} \\ y_{13} \\ \hline  y_{21} \\ y_{22} \\ y_{23}
	\end{bmatrix} 
\end{align}
\end{scriptsize}
Here the horizontal and vertical lines depict the partitioning of the matrices and vectors, possibly on different processors. Hence, the computations can be performed locally for each macro-element in the mesh.

\ 

The final reduction, step 4, can be performed for each macro-element-face in the mesh skeleton
\begin{scriptsize}
\begin{align}
	\begin{bmatrix}
		\hat{w}_1  \\ \hat{w}_2
	\end{bmatrix} =   \underbrace{ 
	\begin{bmatrix}
		 * & * \\ * & *
	\end{bmatrix}}_{C}
	\begin{bmatrix}
		\hat{u}_1  \\ \hat{u}_2
	\end{bmatrix} - 
	\begin{bmatrix}
		\hat{v}_1  \\ \hat{v}_2
	\end{bmatrix}
\end{align}
\end{scriptsize}

\begin{figure}[h!]
	\centering
	\includegraphics[trim = 0cm  0cm 0cm 0cm,clip,width=0.23\textwidth]{figures/hdg_example.pdf}
	\caption{Example discretization for a two macro-element mesh with homogeneous boundary conditions and one macro-element-face.}
\label{fig:hdg}
\end{figure}

\end{example}

\subsection{Setup complete problem}
Let $d\; (=2,3)$, denote the spatial dimension. We assume a structured discretization of the unit cube $[0,1]^d$ into a set of $N = d! \, n^3$ simplicial macro-elements, where $n$ denotes the number of macro-elements in each spatial direction. Every macro-element is divided into a set of $m^{d}$ simplicial $C^0$ finite elements, where $m$ denotes the number of elements per macro-element in each spatial direction. We further assume a polynomial basis on each simplicial element that is of total degree $p$. Below we summarize the defining quantities and the dependent quantities that we use in our analysis.

Defining quantities:
\begin{itemize}
	\item[-] $d$ - spatial dimension ($=2, 3$)
	\item[-] $n$ - number of macro-elements along edge of unit cube $[0,1]^d$
	\item[-] $m$ - number of elements along a macro-element edge 
	\item[-] $p$ - element polynomial order
\end{itemize}


Dependent quantities:
\begin{itemize}
	\item[-] $N = d! \, n^d$ - total number of macro-elements
	\item[-] $M_{(d)} = m^{d}$ - total number of elements per $d$-dimensional macro-element
	\item[-] $Q_{(d)} = \binom{m \, p + d}{d} = \frac{1}{d !} (m\cdot p + 1) \cdots  (m\cdot p + d) < \frac{1}{d!} (m \cdot p + d)^d$ - total number of degrees of freedom per $d$-dimensional macro-element
	\item[-] $D = A_d \, n^d + B_d \, d \, n^{d-1} (n-1)$ where $(A_2=1, B_2=1, A_3=6, B_3=2)$ - number of macro-element faces that make up the mesh skeleton (without boundaries). $A_d$ is the number of shared faces within a cube partitioned by simplices, and $B_d$ is the number of shared faces between two $d$-dimensional cubes.
	\item[-] $d+1$ - number of faces of a $d$-dimensional simplex
	\item[-] $(2p+1)^d$ - upper estimate of the number of non-empty intersections of $C^0$ test and trial functions within one macro-element.
	\item[-] $C^{\text{sparsity}}_{(d)} = \left\{\text{dense arithmetic: } 1,  \text{ sparse arithmetic: } (2p+1)^d / Q_{(d)}\right\}$ - upper estimate of sparsity of the matrices.
\end{itemize}
We recall that the $\binom{n}{k} = \frac{n!}{k! (n-k)!}$ is the binomial coefficient.

We are interested in comparing the hybridized macro-element method for $m > 1$ with the standard HDG-method (choose $m=1$). We assume, and later verify, that a similar level of accuracy can be attained as long as the total number of elements stays equal, that is, $n \cdot m = \text{constant}$.

\subsubsection*{Cost global solver}
The time complexity of the above ``global'' problem can be easily computed. The matrix-vector product can be localized to the macro-element level, that is, on macro-element $k$ the matrix-vector product is,
\begin{enumerate}
	\item $x_{(k)} = B_{(k)}^T \hat{u}_{(k)}$
	\item $y_{(k)} = A_{(k)}^{-1} x_{(k)}$ 
	\item $\hat{v}_{(k)} = B_{(k)} y_{(k)}$
\end{enumerate}
The matrix vector multiplications in step 1 and 3 require at most $\mathcal{O}\left( (d+1) Q_{(d-1)} \cdot Q_{(d)} \right)$ operations. An LU-factorization for $A_{(k)}$ is computed once, which costs $\mathcal{O}\left( Q^3_{(d)} \right)$ operations. Application of the factorization in all subsequent steps costs $\mathcal{O}\left( Q^2_{(d)} \right)$ operations. This means that after the initialization process, one iteration of the solver costs $\mathcal{O}\left( Q^2_{(d)} \right)$ operations.

\begin{remark} The $N = d! \, n^d$ local problems can be run independently, in parallel!
\end{remark}

The final reduction step is performed for each element in the mesh skeleton. Suppose  $\hat{v}_{(l1)}$ and $\hat{v}_{(l2)}$  are the computed vectors associated with the two macro-elements adjecent to face $l$ in the mesh skeleton. Then the reduction step on macro-element face is,
\begin{enumerate}
	\setcounter{enumi}{3}
	\item $\hat{w}_{(l)} = C_{(l)} \hat{u}_{(l)} - \hat{v}_{(l1)} -  \hat{v}_{(l2)}$
\end{enumerate}
The matrix multiplication and subtraction require at most $\mathcal{O}\left( Q^2_{(d-1)} \right)$ operations.

\begin{remark} The $D$ local problems can be run independently, in parallel!
\end{remark}

\begin{remark} Communication happens when parts of $\hat{u}$ are send as input to steps 1-3, and when the output of step 3 is channeled back to perform the reduction in step 4.
\end{remark}

\subsubsection*{Cost local solver}
Once the global problem is solved, that is, the interface degrees of freedom $\hat{u}$ are computed, the local solution can be reconstructed for each macro-element separately, by solving the following problem
\begin{align}
	A_{(k)} u_{(k)} = R_{u(k)} - B^T_{(k)} \hat{u}_{(k)}
	\label{eq:local_matrix_problem}
\end{align}
Again, the computed LU factorization is used, which requires $\mathcal{O}\left( Q^2_{(d)} \right)$ operations. 

\subsection{Memory estimates}
Below we summarize estimates of the required memory for the different submatrices per macroelement in the mesh and macroelement face in the mesh skeleton.
\begin{enumerate}
	\item $B_{(k)}$ - memory storage -  $C^{\text{sparsity}}_{(d)} \cdot (d+1) \cdot Q_{(d-1)} \cdot Q_{(d)} \cdot 8$ bytes  
	\item $A_{(k)} = L_{(k)}U_{(k)}$ - memory storage -  $C^{\text{sparsity}}_{(d)} \cdot Q^2_{(d)} \cdot 8$ bytes
	\item $C_{(l)}$  - memory storage -  $C^{\text{sparsity}}_{(d-1)} \cdot Q^2_{(d-1)} \cdot 8$ bytes
\end{enumerate}
Here we  have assumed double precision arithmetic and $C^{\text{sparsity}}_{(d)} \in (0,1]$ is a constant that denotes the fraction of non-zeros of the associated matrix. Furtermore, we assume that after $A_{(k)}$ is computed, its $LU$-factorization is stored in its place, requiring no additional memory.

The matrices in 1. and 2. are stored for $N$ macro-elements in the mesh, possibly distributed among multiple processors. The matrix in 3. is stored for each of the $D$ macro-element faces in the mesh skeleton, also distributed among multiple processors.

\begin{remark}
For small values of $m$ it is more efficient to use dense linear algebra. However, for higher values of $m$, say $m>10$, sparse solvers may be more efficient. This will depend both on the sparsity of the matrix $A$  (which depends on $m$ and $p$) and the size of the $L1-L2$ cache. (We should benchmark this).
\end{remark}

\subsection{Comparison with HDG}
We are interested in the above estimates of operation counts for different $m,n$ such that $n \cdot m = const$. This case studies the setting where the total number of finite elements are equal. Let $\bar{n}, \bar{m}$ denote the dimensions of $n$ and $m$ for the macro-element HDG method. Then we can compare the number of operations in terms of these parameters for with respect to the standard HDG method, $m = 1$, $n = \bar{m} \cdot \bar{n}$. The results are
\begin{table}[]
\begin{tabular}{lll}
  							& MEHDG 		& HDG 													\\
initialization 	&   $\bar{n}^d (\bar{m} \cdot p + d)^{3d}$    				
							&   $\bar{m}^d \cdot \bar{n}^d (p+d)^{3d}$  				\\
step 1 				&   $\bar{n}^d (\bar{m} \cdot p + d)^{2d-1}$    				
							&   $\bar{m}^d \cdot \bar{n}^d (p + d)^{2d-1}$  		\\
step 2 				&   $\bar{n}^d (\bar{m} \cdot p + d)^{2d}$   				&    
								  $\bar{m}^d \cdot \bar{n}^d (p+d)^{2d}$				\\
step 3 				&   $\bar{n}^d (\bar{m} \cdot p + d)^{2d-1}$    				
							&   $\bar{m}^d \cdot \bar{n}^d (p + d)^{2d-1}$			\\
step 4 				&   $\bar{n}^d (\bar{m} \cdot p + d-1)^{2d-2}$    				
							&   $\bar{m}^d \cdot \bar{n}^d (p + d)^{2d-2}$
\end{tabular}
\caption{Order of operations to initialize one iteration and then perform steps 1 through 4 in every iteration.}
\end{table}





